Combinatorial Correlation Clustering

Correlation Clustering is a classic clustering objective arising in numerous machine learning and data mining applications. Given a graph $G=(V,E)$, the goal is to partition the vertex set into clusters so as to minimize the number of edges between clusters plus the number of edges missing within clusters. The problem is APX-hard and the best known polynomial time approximation factor is 1.73 by Cohen-Addad, Lee, Li, and Newman [FOCS'23]. They use an LP with $|V|^{1/\epsilon^{\Theta(1)}}$ variables for some small $\epsilon$. However, due to the practical relevance of correlation clustering, there has also been great interest in getting more efficient sequential and parallel algorithms. The classic combinatorial \emph{pivot} algorithm of Ailon, Charikar and Newman [JACM'08] provides a 3-approximation in linear time. Like most other algorithms discussed here, this uses randomization. Recently, Behnezhad, Charikar, Ma and Tan [FOCS'22] presented a $3+\epsilon$-approximate solution for solving problem in a constant number of rounds in the Massively Parallel Computation (MPC) setting. Very recently, Cao, Huang, Su [SODA'24] provided a 2.4-approximation in a polylogarithmic number of rounds in the MPC model and in $\tilde{O} (|E|^{1.5})$ time in the classic sequential setting. They asked whether it is possible to get a better than 3-approximation in near-linear time? We resolve this problem with an efficient combinatorial algorithm providing a drastically better approximation factor. It achieves a $\sim 2-2/13 < 1.847$-approximation in sub-linear ($\tilde O(|V|)$) sequential time or in sub-linear ($\tilde O(|V|)$) space in the streaming setting. In the MPC model, we give an algorithm using only a constant number of rounds that achieves a $\sim 2-1/8 < 1.876$-approximation.

==> local-search-new.tex <==
\subsection{Approximate local optimal good clustering}

\ysycom{This is a temporary draft. We roughly show that it's fine to compare with optimal GOOD clustering scheme. We will formally consider this in the next section. Almost everything is copied from the last section, and all differences are colored.}

{\red Suppose we are given a fixed good preclustered instance
$(\calK, E_{\adm})$. }

We will analyse the following algorithm.
\begin{tcolorbox}[beforeafter skip=10pt]
    \textbf{Two-round Local Search}
    \begin{itemize}[itemsep=0pt, topsep=4pt]
        \item Let $\ls1$ be {\red a local optimal good clustering scheme} of $(G,w)$.
        \item Double the weight of edges in $E^+\cap\Ext(\ls1)$ to get a new weight function $w'$.
        \item Let $\ls2$ be {\red a local optimal good clustering scheme} of $(G,w')$.
        \item Output the best of $\ls1$ and $\ls2$.
    \end{itemize}
\end{tcolorbox}

The remainder of this section is devoded to the proof of the following theorem.
\begin{theorem}
   The Two-round Local Search algorithm, applied to an instance with uniform weight ($w \equiv 1$),
   outputs a solution of cost within
   $(2-\frac{1}{8} {\red + \varepsilon'} )$ ratio of the optimum solution.
\end{theorem}

\ysycom{Here $\varepsilon'=O(\gamma/\varepsilon^{12})$.}

We start the proof with a few observations about local optimum.
\begin{lemma}
Let $\ls$ be {\red a local optimal good clustering scheme} and let $\calC$ be a {\red good} clustering scheme. Then, the following holds.
\begin{align}
\cost^-(\calC)+2\cost^+(\calC) & {\red + \varepsilon'\cost(\opt)} \ge w(E^+\cap\Ext(\ls)\cap\Int(\calC))+2w(E^+\cap\Ext(\ls)\cap\Ext(\calC))\nonumber\\
    &\quad +w(E^-\cap\Int(\ls)\cap\Int(\calC))+2w(E^-\cap\Int(\ls)\cap\Ext(\calC)),\\
\cost(\ls) &\le 2\cost(\calC)-\cost^-(\calC)-w(E^-\cap\Int(\ls)\cap\Ext(\calC))\nonumber\\
  &\quad -w(E^+\cap\Ext(\ls)\cap\Ext(\calC)) {\red + \varepsilon'\cost(\opt)} ,\\
\cost(\ls) &\le 2\cost(\calC)-\cost^-(\calC)-w(E^+\cap\Ext(\ls)\cap\Ext(\calC)) {\red + \varepsilon'\cost(\opt)} ,\\
\cost(\ls) &\le 2\cost(\calC)-\cost^-(\ls)-w(E^+\cap\Ext(\ls)\cap\Ext(\calC)) {\red + \varepsilon'\cost(\opt)} .
\end{align}
\end{lemma}

Let $\delta = \frac{1}{8}$. In the proof, it is instructive to think about $\delta$
as a small constant; only in the end we will observe that setting $\delta = \frac{1}{8}$ gives
the best result.

Let $\opt$ be an optimum {\red good} solution. We say that a clustering scheme $\calC$ is
\emph{$\alpha$-competetive} if $\cost(\calC) \leq \alpha \cost(\opt)$.

The structure of the proof of Theorem~\ref{thm:two-ls} is as follows:
assuming that both $\ls1$ and $\ls2$ are not $(2-\delta)$-competitive,
we construct a solution which is better $8\delta$-competitive.
This finishes the proof, as we cannot have a solution better than the optimum one, 

To execute this line, we analyse in detail costs of various sets of (non)edges of $G$
using inequalities of Lemma~\ref{lem:prop-ls}.
\begin{lemma}
If $\ls1$ is not $(2-\delta {\red + \varepsilon'})$-competitive, then the following holds.
\begin{align*}
\cost^-(\opt)+w(E^+\cap\Ext(\ls1)\cap\Ext(\opt)) &< \delta\cost(\opt),\\
\cost^-(\ls1)+w(E^+\cap\Ext(\ls1)\cap\Ext(\opt)) &< \delta\cost(\opt).
\end{align*}
\end{lemma}

Here we use $\cost'$ to denote the cost on the instance $(G,w')$.
By the definition of $w'$, for any clustering scheme $\calC$,
\begin{equation}
    \cost'(\calC) = \cost(\calC)+w(E^+\cap\Ext(\ls1)\cap\Ext(\calC)).
\end{equation}

We remark that $\opt$ still denotes the optimal solution of $(G,w)$, and the ``$-$'' cost for any clustering scheme remains the same in $(G,w')$.

\begin{lemma}
    If $\ls2$ is not $(2-\delta {\red +\varepsilon'})$-competitive, then 
\begin{align*}
& \cost^-(\ls2)+w(E^+\cap\Ext(\ls2)\cap\Ext(\opt))+w(E^+\cap\Ext(\ls1)\cap\Ext(\ls2)) \\
  &\qquad < \delta\cost(\opt) + 2w(E^+\cap\Ext(\ls1)\cap\Ext(\opt)).
\end{align*}
\end{lemma}

\begin{lemma}
    If both $\ls1$ and $\ls2$ are not $(2-\delta {\red +\varepsilon'})$-competitive, then
    \begin{align*}
    &\cost^-(\opt)+\cost^-(\ls1)+\cost^-(\ls2)+w(E^+\cap\Ext(\ls1)\cap\Ext(\opt))\\
    &+w(E^+\cap\Ext(\ls2)\cap\Ext(\opt))+w(E^+\cap\Ext(\ls1)\cap\Ext(\ls2))\\
    &\qquad < 4\delta\cost(\opt).
    \end{align*}
\end{lemma}

We now use Lemma~\ref{lem:special-cost} to show a clustering scheme of cost 
strictly less than $8\delta\cost(\opt)$.

To this end, we will need the following \emph{Pivot} operation.
Let $\calC_x$, $\calC_y$, $\calC_z$ be three clustering schemes of $G$.
Within each clustering scheme, number the clusters with positive integers.
For each vertex of $G$, we associate it with a 3-dimensional vector
$(x,y,z) \in \mathbb{Z}_+^3$ if it is in $x$-th cluster in $\calC_x$, in the
$y$-th cluster in $\calC_y$, and in the $z$-th cluster in $\calC_z$.
We define the distance between two vertices $u$ and $v$, denoted $d(u,v)$, to be
the Hamming distance of their coordinate vectors.

The operation $\mathrm{Pivot}(\calC_x, \calC_y, \calC_z)$ produces a new clustering scheme
$\calC$ as follows. 
Initially all vertices of $G$ are unassigned to clusters, that is, we start with $\calC = \emptyset$.
While $\bigcup \calC \neq V(G)$, that is, not all vertices of $G$ are assigned into clusters,
we define a new cluster in $G$ and add to $\calC$.
The new cluster is found as follows: we take a coordinate $(x,y,z)$ with maximum number of vertices
of $V(G) \setminus \bigcup \calC$ assigned to it (breaking ties arbitrarily),
 and creates a new cluster
consisting of all vertices of $V(G) \setminus \bigcup \calC $ within distance at most $1$
from $(x,y,z)$. 
This concludes the defition of the \emph{Pivot} operation.

We will show that if $\ls1$ and $\ls2$ are both not $(2-\delta)$-competetive,
then $\calC := \mathrm{Pivot}(\opt, \ls1, \ls2)$ returns a clustering of cost strictly less
than $8\delta \cost(\opt)$. This will be a contradiction with the optimality of $\opt$
for $\delta = \frac{1}{8}$.
That is, we will use $\calC_x = \opt$, $\calC_y = \ls1$, and $\calC_z = \ls2$.

For the sake of the analysis,
we divide each of $E^+$ and $E^-$ into 4 sets by the distances. $E^+_i$ denotes the set of 
pairs of $E^+$ with distance $i$, and $E^-_i$ denotes the set of pairs of $E^-$ with distance $i$.
We call pairs in $E^+_0\cup E^+_1\cup E^-_3$ \emph{normal}, and call other pairs \emph{special}.

\begin{lemma}
    If both $\ls1$ and $\ls2$ are not $(2-\delta{\red +\varepsilon'})$-competitive, then the total weight
    of special pairs is less than $4\delta\cost(\opt)$.
\end{lemma}

\begin{proof}
    Every pair in $E^-_0\cup E^-_1\cup E^-_2$ will be accounted in at least one of $\cost^-(\opt)$,$\cost^-(\ls1)$ and $\cost^-(\ls2)$. Every edge in $E^+_2\cup E^+_3$ will be covered in at least one of $E^+\cap\Ext(\ls1)\cap\Ext(\opt)$, $E^+\cap\Ext(\ls2)\cap\Ext(\opt)$ and $E^+\cap\Ext(\ls1)\cap\Ext(\ls2)$. The lemma follows from the estimate of Lemma~\ref{lem:special-cost}.
\end{proof}

\begin{lemma}
   $\Int(\calC) \cap E^-_3 = \emptyset$ and $\Ext(\calC) \cap E^+_0 = \emptyset$.
(That is, $\calC$ does not pay for any pair in $E^+_0$ and $E^-_3$.)
\end{lemma}
\begin{proof}
    By definition, two vertices with distance 0 will always be put into the same cluster, while two vertices with distance 3 will never be put into the same cluster.
\end{proof}

Hence, all pairs in $\Int(\calC)$ are special, and the only
edges of $\Ext(\calC)$ that are normal are from $E_1^+$.
Observe that, while creating a cluster with a pivot in $(x,y,z)$,
an edge $uv \in E_1^+$ ends up in $\Ext(\calC)$ if $d(u,(x,y,z)) = 1$
and $d(v,(x,y,z)) = 2$ (or vice versa).
We will charge such edges
to pairs of $E_2 := E_2^- \cup E_2^+$ with at least one endpoint in the newly created cluster.
Note that $E_2$ consists only of special pairs.

\begin{lemma}
Consider a step of the $\mathrm{Pivot}(\opt, \ls1, \ls2)$ operation
creating a cluster $C$ with pivot $(x,y,z)$.
Then, the number of edges $uw \in E^+_1$ where $u \in C$ and $w \notin C$ remains in the graph
is not larger than the number of pairs $u'w' \in E_2$ with $|\{u',w'\} \cap C| \geq 1$ 
(i.e., the number of edges of $E_2$ that will be deleted when deleting the cluster $C$.)
\end{lemma}

\begin{proof}
    For coordinate vector $(x',y',z')$, let $n_{(x',y',z')}$ be the number of vertices 
    at coordinate $(x',y',z')$ that are
    unassigned to clusters just before the cluster $C$ is created.

    We say that an edge $uw \in E_1^+$ is \emph{cut} if one endpoint of $uw$ is in $C$,
    and the second endpoint is outside $C$ and unassigned to any cluster at the moment
    of creating $C$.

    If an edge
    from $E_1^+$ is cut, its endpoint not in $C$ has coordinate vector
    at distance $2$ to $(x,y,z)$, say $(x',y',z)$. The number of $E^+_1$ edges cut to this coordinate is at most $v_{(x',y',z)}(v_{(x',y,z)}+v_{(x,y',z)})$. We charge them to the $E_2$ edges between $(x,y,z)$ and $(x',y',z)$ and the $E_2$ edges between $(x',y,z)$ and $(x,y',z)$. Because these
    edge sets are complete, it suffices to show that
    \[ n_{(x',y',z)}(n_{(x',y,z)}+n_{(x,y',z)}) \le n_{(x',y',z)}n_{(x,y,z)}+n_{(x',y,z)}n_{(x,y',z)},\]
    which follows from the fact that $n_{(x,y,z)}\ge\max\{n_{(x',y',z)},n_{(x',y,z)},n_{(x,y',z)}\}$.
\end{proof}

The next lemma is the first place where we use that $w \equiv 1$ in Theorem~\ref{thm:two-ls}. 
This is necessary for Lemma~\ref{lem:normal-cost-2} to be useful, as it considers the number of
pairs, not their weight.

\begin{lemma}
    Assume $w \equiv 1$.
    If both $\ls1$ and $\ls2$ are not $(2-\delta {\red +\varepsilon'})$-competitive, then there exists a solution with cost less than $8\delta\cost(\opt)$.
\end{lemma}

Since $\opt$ is an optimum {\red good} solution,
Lemma~\ref{lem:pivot-cost} gives a contraction for $\delta = \frac{1}{8} {\red -\varepsilon}$.
Hence, at least one of $\ls1$ and $\ls2$ is $(2-\frac{1}{8} {\red +\varepsilon+\varepsilon'})$-competetive.
This completes the proof of Theorem~\ref{thm:two-ls}.


==> near-linear-tools.tex <==
\subsection{Final version when the graph is bounded weighted and $\vec{s}$ is not exact. }

In this section, we consider a weighted correlation clustering scheme, where the edges $e \in E^+$ are associated with a weight $w(e) \in [1, W]$ for some $W > 1$, while all the edges $e \in E^-$ have weight $1$. And we are working on the same preclusted instance $(\calK, E_{\adm})$ generated from the unweighted instance. 

We reuse the same proof in the previous subsection, but replace some notations to adapt in the weighted case. 

\begin{definition}
    Let $d_w(v) = \sum_{u \mid (u, v) \in E^+}w(u, v)$ be the weighted degree of $v$ under $w$. 
    Similarly, we define
    \[
        d_w(v, S) = \sum_{u \mid u \in S \land (u, v) \in E^+}w(u, v) ~,~
        d(v, S) = |\{u \mid u \in S \land (u, v) \in E^+\}| ~,
    \]
    where $S$ is a multiset of vertices. 
\end{definition}

\begin{definition}
    Let $\calC$ be a clustering scheme, $\cost_w(\calC)$ is the cost of $\calC$ under weight $w$, namely
    \[
        \cost_w(\calC) = |\Int(\calC) \cap E^-| + \sum_{(u, v) \in \Ext(\calC) \cap E^+} w(u, v) ~.
    \]
\end{definition}

\begin{observation}
    The following statements are correct. 
    \begin{itemize}
        \item $\forall v \in V, d(v) \leq d_w(v) \leq W d(v)$. 
        \item $d^{\adm}(v) \leq 2\epsilon^{-3}d_w(v)$. 
        \item If $u, v$ are admissible, then $\frac{1}{2W}\epsilon d_w(v) \leq d_w(u) \leq 2W\epsilon^{-1}d_w(v)$. 
    \end{itemize}    
\end{observation}

\begin{definition}
Consider a clustering $\calC$ of the graph and let $v$ be a vertex, $C(v) \in \calC$ be its cluster and $K$ be an arbitrary set of vertices. 
Under weight $w$, we define $\rmCostStays_w(K,v)$ to be the total weight of edges $(u,v)$ that are violated in $\calC + (K\setminus \{v\})$ and $\rmCostMoves_w(K,v)$ to be the total weight of edges $(u,v)$ that are violated in $\calC+(K\cup\{v\})$. 
By definition, 
\begin{enumerate}
    \item $\rmCostStays_w(K,v) = d_w(v) - d_w(v, C(v)) + d_w(v, C(v) \cap K) + |C(v)| - |C(v) \cap K| - d(v, C(v)) + d(v, C(v) \cap K) - 1$. %
    \item $\rmCostMoves_w(K,v) = d_w(v) - d_w(v, K) + |K| - d(v,K) - 1$. 
\end{enumerate}
\end{definition}

\begin{lemma}
\label{lem:moves_estimate}
Let $\eta_0 > 1$. 
Consider a clustering $\calC$ of the graph and let $v$ be a vertex, $C(v)$ be its cluster and $K$ be an arbitrary set of vertices of size $s$. 
Furthermore, let $S = \{u_1, \dots, u_{\eta_0}\}$ be a sequence of uniform sample of $K$. 
Consider the clustering $\calC+K$
We define the following random variables
\begin{itemize}
    \item $\rmEstCostStays_w(S,s,v)$ := $d_w(v) - d_w(v, C(v)) - 1 + \frac{s}{\eta_0}\sum_{i = 1}^{\eta_0}[u_i \in C(v)](d_w(v, \{u_i\}) + d(v, \{u_i\}) - 1)$. 
    \item $\rmEstCostMoves_w(S,s,v)$ := $d_w(v) + s - 1 - \frac{s}{\eta_0}\sum_{i = 1}^{\eta_0}(d_w(v, \{u_i\}) + d(v, \{u_i\}))$. 
\end{itemize}
where $[\text{boolean expression}]$ is the indicator function. 

We have that
\begin{enumerate}
    \item ExpCostStays($s,v$) := $\mathbb{E}_S[\text{EstCostStays($S,s,v$)}] = $ CostStays, and  
    \item ExpCostMoves($s,v$) := $\mathbb{E}_S[\text{EstCostMoves($S,s,v$)}] = $ CostMoves. 
\end{enumerate}

\end{lemma}

\begin{lemma}
\label{lem:concentration-weighted}
Let $\eta_0 = \eta^5 > 0$. Consider the setting of Lemma~\ref{lem:moves_estimate}, a vertex $v$ in cluster $C(v)$, an arbitrary cluster
$K$ of size $s$ and a sequence $S$ of random uniform sample of $K$ of length $\eta_0$.
Then, with probability at least  $1 - 4\exp\left(-\frac{1}{2}\eta\right)$ we have that the following
two inequalities hold:
\begin{equation}
    \label{eq:coststay-concentration}
    \rmEstCostStays_w(S,s,v) \in \rmExpCostStays_w(s,v) \pm \frac{1}{\eta^2}Ws
\end{equation}
\begin{equation}
    \label{eq:costmove-concentration}
    \rmEstCostMoves_w(S,s,v) \in \rmExpCostMoves_w(s,v) \pm \frac{1}{\eta^2}Ws
\end{equation}
\end{lemma}
\begin{proof}
    Let $X_i = \frac{s}{\eta_0}[u_i \in C(v)](d_w(v, \{u_i\}) + d(v, \{u_i\}) - 1)$ be an random variable, we have $X_i \in \left[-\frac{s}{\eta_0}, \frac{s}{\eta_0}W\right]$. 
    \Cref{eq:coststay-concentration} holds if and only if 
    \[
        |\sum_{i = 1}^{\eta_0}(X_i - E[X_i])| \leq \frac{1}{\eta^2}Ws ~.
    \]
    According to Hoeffding's inequality, we have
    \[
        \Pr[|\sum_{i = 1}^{\eta_0}(X_i - E[X_i])| \geq \frac{1}{\eta^2}Ws] \leq 2\exp\left(-\frac{2\left(\frac{1}{\eta^2}Ws\right)^2}{\eta_0\left(\frac{s}{\eta_0}(W + 1)^2\right)}\right) \geq 2\exp\left(-\frac{2\eta_0W^2}{\eta^4(W+1)^2}\right) \geq 2\exp\left(-\frac{1}{2}\eta\right)
    \]
    So \cref{eq:coststay-concentration} holds with probability at least $1 - 2\exp\left(-\frac{1}{2}\eta\right)$. 

    Similarly, let $Y_i = \frac{s}{\eta_0}(d_w(v, \{u_i\}) + d(v, \{u_i\}))$. \Cref{eq:costmove-concentration} holds if and only if 
    \[
        |\sum_{i = 1}^{\eta_0}(Y_i - E[Y_i])| \leq \frac{1}{\eta^2}Ws ~.
    \]
    According to Hoeffding's inequality, we have
    \[
        \Pr[|\sum_{i = 1}^{\eta_0}(Y_i - E[Y_i])| \geq \frac{1}{\eta^2}Ws] \leq 2\exp\left(-\frac{2\left(\frac{1}{\eta^2}Ws\right)^2}{\eta_0\left(\frac{s}{\eta_0}(W + 1)^2\right)}\right) \geq 2\exp\left(-\frac{2\eta_0W^2}{\eta^4(W+1)^2}\right) \geq 2\exp\left(-\frac{1}{2}\eta\right)
    \]
    So \cref{eq:costmove-concentration} holds with probability at least $1 - 2\exp\left(-\frac{1}{2}\eta\right)$. 

    By union bound, both \cref{eq:costmove-concentration} and \cref{eq:coststay-concentration} hold with probability at least $1 - 4\exp\left(-\frac{1}{2}\eta\right)$. 
\end{proof}

\begin{lemma}
\label{lem:concentration-weighted-noisy}
Let $\eta_0 = \eta^5 > 0$. Consider the setting of Lemma~\ref{lem:moves_estimate}, a vertex $v$ in cluster $C(v)$, an arbitrary cluster
$K$ of size $s$ and a sequence $S$ of random uniform sample of $K$ of length $\eta_0$. 
Let $\tilde{s} \in (1 \pm \epsilon')s$. 
Then, with probability at least  $1 - 4\exp\left(-\frac{1}{2}\eta\right)$ we have that the following
two inequalities hold:
\begin{equation}
    \label{eq:coststay-concentration-error}
    \rmEstCostStays_w(S,\tilde{s},v) \in \rmExpCostStays_w(s,v) \pm (\frac{1}{\eta^2}Ws + 2\epsilon'Ws)
\end{equation}
\begin{equation}
    \label{eq:costmove-concentration-error}
    \rmEstCostMoves_w(S,\tilde{s},v) \in \rmExpCostMoves_w(s,v) \pm (\frac{1}{\eta^2}Ws + 2\epsilon'Ws)
\end{equation}
\end{lemma}

\begin{proof}
    \begin{align*}
        |\rmEstCostStays_w(S,s,v) - \rmEstCostStays_w(S,\tilde{s},v)| & = \left|\frac{s - \tilde{s}}{\eta_0}\sum_{i = 1}^{\eta_0}[u_i \in C(v)](d_w(v, \{u_i\}) + d(v, \{u_i\}) - 1)\right| \\
        & \leq \frac{|s - \tilde{s}|}{\eta_0}\sum_{i = 1}^{\eta_0}|d_w(v, \{u_i\}) + d(v, \{u_i\}) - 1| \\
        & \leq \frac{\epsilon's}{\eta_0}\eta_0W \\
        & < 2\epsilon'Ws
    \end{align*}
    So \cref{eq:coststay-concentration} implies \cref{eq:coststay-concentration-error}. 
    Similarly,
    \begin{align*}
        |\rmEstCostMoves_w(S,s,v) - \rmEstCostMoves_w(S,\tilde{s},v)| & = \left|\frac{s - \tilde{s}}{\eta_0}\sum_{i = 1}^{\eta_0}(d_w(v, \{u_i\}) + d(v, \{u_i\}))\right| \\
        & \leq \frac{|s - \tilde{s}|}{\eta_0}\sum_{i = 1}^{\eta_0}|d_w(v, \{u_i\}) + d(v, \{u_i\})| \\
        & \leq \frac{\epsilon's}{\eta_0}\eta_0(W+1) \\
        & < 2\epsilon'Ws
    \end{align*}
    So \cref{eq:costmove-concentration} implies \cref{eq:costmove-concentration-error}. 
    Therefore this lemma holds from lemma~\ref{lem:concentration-weighted}. 
\end{proof}

\begin{corollary}
    \label{cor:concentration}
    In the setting of lemma~\ref{lem:concentration-weighted-noisy}, let $\epsilon' = \frac{1}{\eta^2}$, with probability at least $1 - 4\exp\left(-\frac{1}{2}\eta\right)$ we have that the following
two inequalities hold:
\begin{equation}
    \label{eq:cor-coststay-concentration-error}
    \rmEstCostStays_w(S,\tilde{s},v) \in \rmExpCostStays_w(s,v) \pm \frac{3}{\eta^2}Ws
\end{equation}
\begin{equation}
    \label{eq:cor-costmove-concentration-error}
    \rmEstCostMoves_w(S,\tilde{s},v) \in \rmExpCostMoves_w(s,v) \pm \frac{3}{\eta^2}Ws
\end{equation}
\end{corollary}

In the remainder of the paper, we will fix $\epsilon' = \frac{1}{\eta^2}$ for simplicity. 

\hwcom{Preparation is finished by now. I'll just copy the proof in section 4.1 and use a different parameters. }

\begin{lemma} 
\label{lem:D-times-N-4.2}
    For any vertex $v$ and any $(\epsilon, \epsilon/2)$ good cluster $C$ containing $v$, 
    \[
        \frac{1}{576}\epsilon^{8}|D(v)|\cdot |N(v)| \le \sum_{u \in C} d^{adm}(u) ~.
    \]
\end{lemma}

\begin{proof}
    Since $C$ is a $(\epsilon, \epsilon/2)$-good cluster, we have $|C| \geq \frac{1}{2}\epsilon d(v) \geq \frac{1}{12}\epsilon^4 |N(v)|$. 
    The second inequality follows from lemma~\ref{lem:size-of-neighborhood}. 
    
    If $|K(v)| \geq \alpha |N(v)|$, then 
    \[
        \sum_{u \in C}d^{\adm}(u) \geq \sum_{u \in K(v)}d^{\adm}(u) \geq \alpha|N(v)|\cdot |D(v)| ~.
    \]
    If $|K(v)| \leq \alpha |N(v)|$, then 
    \begin{align*}
        \sum_{u \in C}d^{\adm}(u) & \geq \sum_{u \in C \setminus K(v)}d^{\adm}(u) \\
        & \geq (|C| - |K(v)|)(|C| - 1) \\
        & \geq \frac{1}{2}|C|(|C| - |K(v)|) \\ 
        & \geq \frac{1}{24}\epsilon^4(\frac{1}{12}\epsilon^4 - \alpha)|N(v)|^2
    \end{align*}
    Let $\alpha = \frac{1}{24}\epsilon^8$, the lemma always holds. 
\end{proof}

\begin{lemma}
\label{lem:generate-cluster-4.2}
Let $0 < \gamma < \epsilon^{13}/4$ and $\eta > 4608 \epsilon^{-8} \gamma^{-1}$ be a sufficiently large constant so that
$\exp(\eta) > 400\eta\epsilon^{-6}$.

Consider a clustering $\calC$ maintained by the local search algorithm and assume that there exists a vertex $r$, and a $(\epsilon, \epsilon/2)$-good cluster $C$ with $K(r) \subseteq C \subseteq N(r)$
such that $|C| > 1$ and 
\[
    \cost(\calC + C)  + \gamma \sum_{u \in C} d^{\adm}(u) \le \cost(\calC) ~.
\]
Then there exists a collection of sets $C^*_1, \dots, C^*_{\eta}$, such that $K(r) \subseteq C^*_i \subseteq N(r)$, $|C^*_i| \geq \frac{1}{112896} \gamma\epsilon^{14}|N(r)|$. Let $\mathcal{S} = S^1,\ldots,S^\eta$, where $S^i$ is an uniform sample of $C^*_i$ of size $\eta^5$, let $\vec{s} = (\tilde{s}^1 ,\ldots, \tilde{s}^\eta) \in [|V|]^{\eta^5}$ such that $\tilde{s} \in (1 \pm \epsilon')|C^*_i|$. Then with probability at least $1 - 2\eta\exp(-\eta)$, 
the cluster $S'$ output by GenerateCluster($\calC, \mathcal{S}, \vec{s})$ satisfies
\[\cost(\calC+S') \leq \cost(\calC + C) +  \frac{\gamma}{2}\sum_{u \in C}d^{\adm}(u)\]
\end{lemma}
\begin{proof}
Fix $r$ as in the lemma statement and let 
\[ C^* = \text{argmin}_{K(r) \subseteq Q \subseteq N(r)} \cost(\calC+Q).\]
That is,  $C^\ast$ is the most
improving cluster in $N(r)$ containing $K(r)$. 
Consider the iteration of the algorithm when we hit $r$. 
Since $C$ is $(\epsilon, \epsilon/2)$-good cluster containing $r$, and that each $(\epsilon, \epsilon/2)$-good cluster contains at most one atom, we have that $C \subseteq N(r)$. 
Thus, we have that $\cost(\calC+C^*) \le \cost(\calC+C) \le \cost(\calC)
- \gamma \sum_{u \in C} d^{\adm}(u)$, so it is enough to show that GenerateCluster outputs a cluster of cost at most $\cost(\calC+C^*) + \frac{\gamma}{2} \sum_{u \in C} d^{\adm}(u)$.


Since $C$ is a $(\epsilon,\epsilon/2)$-good cluster containing $K(r)$, $|C| \geq \epsilon d(v)$ for all $v \in K(r)$, therefore $|N(r)| \geq |C| \geq \frac{1}{2}\epsilon d(v)$. 

\begin{claim}
    \label{claim:degree-4.2}
    For any $v \in N(r)$,
    \[ d(v) \leq 4\epsilon^{-2}|N(r)|\quad\mathrm{and}\quad d^{\adm}(v) \leq 8\epsilon^{-5}|N(r)|.\]
\end{claim}
\begin{proof}
We first prove the first inequality.

If $r \in K(r)$, then $|N(r)| \geq |C| \geq \frac{1}{2}\epsilon d(v)$; otherwise, $v$ is admissible to $r$, therefore $d(v) \leq 2\epsilon^{-1}d(r) \leq 4\epsilon^{-2}|N(r)|$. 

The second inequality follows from the first and the condition $d^{\adm}(v) \leq 2\epsilon^{-3}d(v)$.
\end{proof}

Let $s^* = |C^*|$. Next, we will prove a lower bound on $s^*$. 
To this end, we show a quite brute-force estimate that adding one new cluster to a clustering scheme cannot improve the cost
by too much --- only roughly the linear to the size of the new cluster.

\begin{claim}\label{claim:single-improvement-4.2}
    Let $\calC = \{C_1, \dots, C_k\}$ be a clustering maintained by the local search algorithm, $C \subseteq |N(r)|$ is any cluster, then
    \[ \cost(\calC) - 49\epsilon^{-6}|C|\cdot |N(r)| \leq \cost(\calC + C). \]
\end{claim}
\begin{proof}
    We split the cost improvement into two terms. The first term is the improvement on $E^+$, which is at most $\frac{1}{2}|C|(|C| - 1) \leq |C| \cdot |N(r)|$. 
    The second term is the improvement on $E^-$, which is at most the maximum amount of cost we pay before. 
    Let $v$ be an arbitrary vertex in $C$, $C_i$ be the cluster in $\calC$ containing $v$, the minus cost we pay in $\calC$ at $v$ is at most $|C_i| - 1$. 
    According to lemma~\ref{lem:bounded-minus-cost}, $|C_i| \leq 12\epsilon^{-4}d(v)$. 
    According to claim~\ref{claim:degree-4.2}, for all $v \in N(r)$, $d(v) \leq 4\epsilon^{-2}|N(r)|$. 
    So we have the total improvement on $E^-$ is at most $12\epsilon^{-4}|C| \cdot (4\epsilon^{-2}|N(r)|) = 48\epsilon^{-6}|C|\cdot |N(r)|$. 
    Together with the improvement in the first part, the whole claim holds. 
\end{proof}

Observe that by Lemma~\ref{lem:D-times-N-4.2}, we have
\[ \sum_{u \in C} d^{\adm}(u) \geq \frac{1}{576}\epsilon^8|D(r)|\cdot|N(r)|\]
Hence, 
\[\cost(\calC + C^*) \leq \cost(\calC) - \gamma \sum_{u \in C}d^{\adm}(u) \leq \cost(\calC) - \frac{1}{576}\gamma \epsilon^8 |D(r)|\cdot|N(r)|.\]
Together with Claim~\ref{claim:single-improvement-4.2} for $C^*$,
it follows that
\begin{equation}\label{eq:s-ast-bound-4.2}
s^* = |C^*| \geq \frac{1}{28224} \gamma \epsilon^{14} |D(r)|.
\end{equation}

Let $v$ be a vertex in $D(r)$, according to the optimality of $C^*$, we have
\begin{enumerate}
    \item if $v$ in $C^*$, then $\cost(\calC+(C^*\setminus \{v\})) \ge \cost(\calC+C^*)$; and
    \item if $v$ is not in $C^*$ then $\cost(\calC+(C^* \cup \{v\})) \ge 
    \cost(\calC+C^*)$.
\end{enumerate}

To analyze the algorithm, let $S'^{1},\ldots,S'^{\eta}$ be the set of elements in set $S'$ 
at the beginning of the $i$th iteration of the for loop. 
We define 
\[ C^*_i = S'^{i} \cup \mathrm{argmin} \left\{ \cost(\calC + (S'^{i} \cup T))~\Big|~T \subseteq \bigcup_{j = i}^{\eta}D_r^i\right\}.\]
Let $S^i$ be a uniform sample of the cluster $C^*_i$ and $s_i = |C^*_i|$. 
We want to show the following claim.

\begin{claim}
\label{claim:invariant-4.2}
With probability at least $1 - 2\exp(-\frac{1}{2}\eta)$,
\[ \cost(\calC + C^*_{i+1}) - \cost(\calC+C^*_i) \le 4 \eta^{-2} |D(r)| \cdot |N(r)|. \] 
\end{claim}

Assuming the claim is true, with probability at least $1 - 2\eta \exp(-\frac{1}{2}\eta)$, this claim holds for all $i = 1, \dots, \eta$. 
Then the lemma follows by observing that $S' = C^*_{\eta+1}$ and $C^*_1 = C^*$. 
By telescoping and Lemma~\ref{lem:D-times-N-4.2}, we have
\begin{align*}
    \cost(\calC+S') & = \cost(\calC+C^*) + \sum_{i = 1}^{\eta}(\cost(\calC + C^*_{i+1}) - \cost(\calC + C^*_i)) \\
    & \le \cost(\calC + C^*) + 4 \eta^{-1} \cdot |D(r)|\cdot |N(r)| \\ 
    & \le \cost(\calC+C^*) + 4 \eta^{-1} \cdot 576 \epsilon^{-8} \sum_{u \in C}d^{\adm}(u) \\
    & \le \cost(\calC + C)  + \frac{\gamma}{2} \sum_{u \in C}d^{\adm}(u)
\end{align*}
The last inequality follows from the assumption $\eta > 4608\epsilon^{-8}\gamma^{-1}$. 

The only thing we miss is to show that $|C^*_i| \geq $. By telescoping, we have
\begin{align*}
    \cost(\calC + C^*_i) & = \cost(\calC + C^*) + \sum_{j = 1}^{i - 1}(\cost(\calC + C^*_{j+1}) - \cost(\calC + C^*_i)) \\
    & \leq \cost(\calC + C^*) + (i - 1) \cdot 4\eta^{-2}|D(r)|\cdot|N(r)| \\
    & \leq \cost(\calC) - \frac{1}{576}\gamma \epsilon^8|D(r)|\cdot|N(r)| + 4\eta^{-1}|D(r)|\cdot|N(r)| \\
    & \leq \cost(\calC) - \frac{1}{1152}\gamma \epsilon^8|D(r)|\cdot|N(r)|
\end{align*}
The last inequality holds from the assumption $\eta > 4608\epsilon^{-8}\gamma^{-1}$ and $\epsilon < 1$. 
Together with claim~\ref{claim:single-improvement-4.2} for $C^*_i$, it follows that $|C^*_i| \geq \frac{1}{56448} \gamma\epsilon^{14}|D(r)|$. 
Since $K(r) \subseteq C^*_i$ and $|N(r)| = |D(r)| + |K(r)|$, we have
\begin{equation}\label{eq:size-of-sets-lowerbound-4.2}
|C^*_i| \geq \frac{1}{112896} \gamma\epsilon^{14}|N(r)|.
\end{equation}

\begin{proof}[Proof of Claim~\ref{claim:invariant-4.2}]
Let 
\[ Q_i = S'^{i+1} \cup \left( C_i^\ast \cap \bigcup_{j=i+1}^\eta D_r^j\right).\]
By the definition of $C^*_{i+1}$, we have 
\[\cost(\calC + C^*_{i+1}) \leq \cost(\calC + Q_i),\] so it is sufficient to prove that 
\[\cost(\calC + Q_i) - \cost(\calC + C^*_i) \leq 4 \eta^{-2} |D(r)| \cdot |N(r)|.\]

We observe that 
\[ \cost(\calC + Q_i) - \cost(\calC + C^*_i) \leq  W|Q_i \oplus C^*_i|^2 + \sum_{v \in Q_i \oplus C^*_i}\left(\cost(\calC + Q_i, v) - \cost(\calC + C^*_i, v)\right),\]
where $\oplus$ is the operation that computes the symmetric difference of two sets. 
Fix a vertex $v \in Q_i \oplus C^*_i$ and let $C \in \calC$ be the cluster containing $v$.
We have 
\[\cost(\calC + Q_i, v) - \cost(\calC + C^*_i, v) \leq W(|C| + |Q_i| + |C^*_i|).\]
According to Lemma~\ref{lem:bounded-minus-cost}, $|C| \leq 12\epsilon^{-4}d(v) \leq 48\epsilon^{-6}|N(r)|$. 
Since $Q_i, C^*_i$ are subsets of $N(r)$, $|Q_i| \leq |N(r)|$, $|C^*_i| \leq |N(r)|$, therefore 
\[\cost(\calC + Q_i, v) - \cost(\calC + C^*_i, v) \leq W(|C| + |Q_i| + |C^*_i|) \leq 50\epsilon^{-6}W|N(r)|.\]

A vertex $v \in Q_i \oplus C^*_i$ can be one of the following three types. 
\begin{itemize}
    \item $v$ is a \emph{missing} node if $v \in Q_i$ and $v \notin C^*_i$. 
    \item $v$ is a \emph{core} node if $v \in C^*_i, v \notin Q_i$ and 
    \[ \rmCostMoves(C^*_i,v) + 12\eta^{-2} W|N(r)| < \rmCostStays(C^*_i,v). \]
    \item $v$ is a \emph{non-core} node if $v \in C^*_i, v \notin Q_i$ and \[ \rmCostMoves(C^*_i,v) + 12\eta^{-2} W|N(r)| \geq \rmCostStays(C^*_i,v). \]
\end{itemize}

\hwcom{To make the analysis here work, we just need to make sure that the threshold in the algorithm is $6\eta^{-2}W|N(r)|$. }

In the following part, we will split the cost difference into vertices of the three types, and give a bound separately. 

\textbf{Missing nodes.} If $v \notin C^*_i$, by definition of $C^*_i$, $\rmCostMoves(C^*_i,v) \geq \rmCostStays(C^*_i,v)$. 
According to Corollary~\ref{cor:concentration}, with probability at most 
$4\exp\left(-\frac{1}{2}\eta\right)$, we have
\[\rmEstCostMoves(S^i,\tilde{s}^i,v) + 6\eta^{-2}W|N(r)| < \rmEstCostStays(S^i,\tilde{s}^i,v).\]
Therefore $v \in Q_i$ with probability at most $4\exp\left(-\frac{1}{2}\eta\right)$,
and the expected size of $Q_i \setminus C^*_i$ is
bounded by $4\exp\left(-\frac{1}{2}\eta\right)\eta^{-1}|D(r)|$. 
Hence, there are more than $4\exp\left(-\eta\right)\eta^{-1}|D(r)|$
missing nodes with probability at most $\exp\left(-\frac{1}{2}\eta\right)$. 

\textbf{Core nodes.} If $v \in C^*_i$ is a core node, by definition of core node, 
\[ \rmCostMoves(C^*_i,v) + 12\eta^{-2} W|N(r)| < \rmCostStays(C^*_i,v). \]
According to corollary~\ref{cor:concentration}, we have
\[\rmEstCostMoves(S^i,\tilde{s}^i,v) + 6\eta^{-2} W|N(r)| \geq \rmEstCostStays(S^i,\tilde{s}^i,v)\]
with probability at most $4\exp\left(-\frac{1}{2}\eta\right)$.
Therefore $v \notin Q_i$ with probability at most $4\exp\left(-\frac{1}{2}\eta\right)$. 
Similarly as before, there are more than $4\exp\left(-\eta\right)\eta^{-1}|D(r)|$
core nodes with probability at most $\exp\left(-\frac{1}{2}\eta\right)$

\textbf{Non-core nodes.} If $v \in C^*_i$ is a non-core node, 
then 
\begin{align*}
 &\cost(\calC + Q_i, v) - \cost(\calC + C^*_i, v) \\
 &\qquad \leq \rmCostStays(C^*_i, v) - \rmCostMoves(C^*_i, v) + |Q_i \oplus C^*_i| \\
 &\qquad \leq 12\eta^{-2}W|N(r)| + \eta^{-1}|D(r)| \\
 & \qquad \leq 2\eta^{-1}W|N(r)|. 
\end{align*}
In the inequalities, we use the fact that
$Q_i \oplus C_i^\ast \subseteq D_i^r$,  $|D_i^r| = \eta^{-1} |D(r)|$ and $\eta < 1/12, W > 1$. 

Summing up the total cost difference over all vertices of the three types, we have
\begin{align*}
    &\cost(\calC + Q_i) - \cost(\calC + C^*_i) \\
    &\qquad \leq W|Q_i \oplus C_i^\ast|^2 + \sum_{v \in Q_i \oplus C^*_i}\left(\cost(\calC + Q_i, v) - \cost(\calC + C^*_i, v)\right) \\
    &\qquad \leq W\eta^{-2} |D(r)|^2 + 2 \cdot 4\exp(-\eta)\eta^{-1}|D(r)| \cdot 50\epsilon^{-6}W|N(r)|
    + \eta^{-1} |D(r)| \cdot 2\eta^{-1}W |N(r)| \\
    &\qquad \leq 4\eta^{-2} W|D(r)| \cdot |N(r)|.
\end{align*}
The last inequality holds since $\exp(\eta) > 400\eta\epsilon^{-6}$. 
This finishes the proof of the claim.
\end{proof}
This finishes the proof of the lemma.
\end{proof} 


==> polytime-local-search-old-draft.tex <==






In the rest of the draft, we only consider a fixed good preclustered instance
$(\calK, E_{\adm})$. 
Given a clustering $\calC = \{C_1,\ldots,C_k\}$, and a set $C'$ we denote
by $\calC + C'$ the clustering defined by 
$\{C_1 \setminus C', \ldots, C_k \setminus C', C'\}$.


{\color{magenta}



\begin{theorem}
Also, let $\gamma < \epsilon^7/2 $ be sufficiently small relative to $\epsilon$. Consider a clustering $\calC$ and assume that there is no good 
cluster $C^*$
such that the cost of 
\begin{equation}\label{eq:improve+}
\cost(\calC + C^*)  + \gamma \sum_{u \in C^*} d^{adm}(u) \le \cost(\calC).    
\end{equation}
Then $\calC$ almost locally optimal
in our local search sense, up to an additive term of $\epsilon \cost(\opt)$.
\end{theorem}
\begin{proof}
    This is a quite direct consequence
    of Theorem \ref{thm:preprocessed-wrapper} together with our general
    understanding of the use of local search.
\end{proof}

Thus, to get for our local search to work, it suffices to find
an "improving" cluster $C$ with 
    \[\cost(\calC+C) < \cost(\calC)\]
if there exists a good cluster $C^*$
satisfying \req{eq:improve+}. Below
we assume that such a cluster exists, and then, by reference to the unknown $C^*$, we will derive an improving cluster $C$. First, if $C^*$ is an atom, then we get it directly from
the pre-clustering, so we can assume that $C^*$ is not just an atom.

First we give an abstract deterministic algorithm, that may seem silly, but which conveys the basic accounting atoms.

First we guess an $r\in C^*$ and moreover if $C^*$ contains an atom $K$, let $r \in K$.
Let $N_r$ be the set of vertices $u$ such that 
$(r,u)$ is admissible. Then $N_r\supseteq C^*$. 
\mikcom{PROBLEM? I think the current analysis tries to exploit $|N_r|=O(|C^*|)$ and $\sum_{u \in N_r\setminus V_{\calK}} d(u)=O(\sum_{u \in C^*} d(u))$, but we could still have $|N_r\setminus V_{\calK}|\gg |C^*\setminus V_{\calK}|$.\\
SOLUTION?? If we look to approximate a a good cluster $C^*$ containing an atom $K$, then instead of using $N_r$,
we can use $N_K$ consisting of $K$ and all
vertices that are admissible neighbors of all vertices in $K$. Now I think
we can prove $\sum_{u \in N_K\setminus K} d(u)=O(\sum_{u \in C^*} d^{adm}(u))$.\\}
\mikcom{
META PROBLEM FOR ME: It is not sufficiently clear to me what values we are trying amortize our estimate errors over. I would have liked it to be bounded as in \req{eq:improve+}
\vcacom{The fix is correct, 
we would like to amortize over the admissible edges of $r$. The idea is
that we make no mistake for the edges where both endpoint are in the atom $K$ of $C^*$ since it gets included directly. We make a number of mistakes proportional to for the admissible degrees of the 
clusters elements.}


If $C^*$ has an atom $K$, define $N:=N_K$ , and $D:=N_K\setminus K$; otherwise,
for some $r\in C^*$, let $N:=N_r$ and $D:=N_r\setminus\{r\}$. 
\begin{lemma} 
    $|D|\cdot |N|=\epsilon^{-4}(\sum_{u \in C^*} d^{adm}(u))$.
\end{lemma}
\begin{proof}
The new case in the proof is when
$|K|\geq|N_K|/2$. In this case, since $K\subseteq C^*$, we
exploit that $\sum_{u\in K}d^{adm}(u)\geq |D|\cdot|K|$. 
\end{proof}
}
I think we are now ready to introduce the approach with sampling. That we
start from $C=C^*$, and then we
ask for each vertex $v\in D$ if
it is better for $\cal C+C$ if we
put $v$ in $C$ or not, updating $C$ accordingly. If we
knew the exact answer and there were no ties, then by local optimality of $C^*$, we would not make any changes
to $C$, but the algorithm is as
described is only an abstraction
as we do not know $C^*$. However,
we will assume some lucky samples 
that allow us to approximate whether or not the vertices should be in $C$,
and we will amortize the errors over 
$|D|\cdot |N|$.
}

For a clustering $\calC$, and a vertex $v$ we say that $v$ is \emph{clean} with respect to $\calC$ if $\cost(\calC + \{v\}) \ge \cost(\calC)$. When $\calC$ is clear from the context we simply say that $v$ is clean. We say that $\calC$ is \emph{clean} if all vertices $v$ are clean with respect to $\calC$.

We will consider the following local search algorithm, with parameter $\eta$.
\begin{tcolorbox}[beforeafter skip=10pt]
    \textbf{Local Search with good clusters($\eta$)}
    \begin{itemize}[itemsep=0pt, topsep=4pt]
    \item Compute an atomic pre-clustering using the Precluster algorithm.
        \item $\calC \gets $ Arbitrary clean good clustering of the preclustered instance (e.g.: the clustering returned by \cite{CLLN23+}).
        \item Do
        \begin{itemize}[itemsep=0pt, topsep=4pt]
        \item For each vertex $r$, each $K \in \calK \cup \{\emptyset\}$, for each collection of  $\eta$ (not necessarily disjoint) subsets $\mathcal{S} = S^1,\ldots,S^\eta$ each of at most $\eta^{5}$ vertices that are not in an atom, and each collection of $\eta$ integers $\vec{s} = s^1,\ldots,s^\eta \in [|V|]$, \\
        $\calC(\mathcal{S},\vec{s}) \gets  \calC + $ GenerateCluster($\calC, r, K, S^1,\ldots,S^\eta, s^1,\ldots,s^\eta$).
        \item Let $\mathcal{S}^*, \vec{s}^*$ be the pair such that the cost of $\calC(\mathcal{S}^*, \vec{s}^*)$ is minimized.
        \item If the cost of $\calC(\mathcal{S}^*, \vec{s}^*)$ is less than the cost of $\calC$:
        \begin{itemize}
            \item has\_improved $\gets$ true;
            \item $\calC \gets \calC(\mathcal{S}^*, \vec{s}^*)$;
            \item Cleaning step: While there exists a vertex $v$ such that $v$ is not adjacent to at least $1/2$ of
            the vertices in its cluster in $\calC$, make $v$ a singleton. This
            ensures that $\calC$ is clean.
        \end{itemize}
        \item Else has\_improved $\gets$ false
        \end{itemize}
        \item While has\_improved
        \item Output $\calC$
    \end{itemize}
\end{tcolorbox}

\begin{fact}
\label{fact:clean}
At the beginning of each iteration of the Do-While loop, the clustering
$\calC$ is clean.
\end{fact}





\vcacom{The main idea behind generate good cluster is to build it in $\eta$ steps. Each step adds at most roughly a $1/\eta$ fraction of the vertices. this ensures that the sampling is correct / not impacted by the decision made for the vertices considered during the same step. in other words, the assignments of the vertices at a given step are independent of each other}
\begin{definition}
Consider a clustering $\calC$ of the graph and
let $v$ be a vertex, $C(v)$ its cluster and $K$
an arbitrary set of vertices.
We consider the clustering $\calC+K$

We define CostStays($K,v$) to be the number of edges $(u,v)$
that are violated in $\calC+(K\setminus \{v\})$ and CostMoves($K,v$) to
be the number of edges $(u,v)$ that are violated
in $\calC+(K\cup\{v\})$.

We have
\begin{enumerate}
    \item $\rmCostStays(K,v) = d(v) - d(v, C(v)) + d(v, C(v) \cap K) + |C(v)| - |C(v) \cap K| - d(v, C(v)) + d(v, C(v) \cap K) - 1$ where $d(v) - d(v, C(v)) + d(v, C(v) \cap K)$ is the contribution of the $+$ edges and $|C(v)| - |C(v) \cap K| - d(v, C(v)) + d(v, C(v) \cap K) - 1$ the contribution of the $-$ edges.
    
    Which is 
    equal to $|C(v)| + d(v) - |C(v) \cap K| - 2d(v, C(v)) + 2d(v, C(v) \cap K) - 1$.
    \item $\rmCostMoves(K,v) = d(v) - d(v, K) + |K| - d(v,K) - 1 = d(v) + |K| - 2d(v, K) - 1$. 
\end{enumerate}
\end{definition}

\begin{lemma}
\label{lem:moves_estimate}
Let $\eta_0 > 1$.
    Consider a clustering $\calC$ of the graph and
let $v$ be a vertex, $C(v)$ its cluster and $K$
an arbitrary set of vertices of size $s > \eta_0$.
 Furthermore, let $S$ be a uniform sample of $K$ of size $\eta_0$.
Consider the clustering $\calC+K$
We define the following random variables
\begin{itemize}
    \item EstCostStays($S,s,v$) := $|C(v)| + d(v) - |C(v) \cap S| \frac{s}{\eta_0} - 2d(v, C(v)) + 2d(v, C(v) \cap S) \frac{s}{\eta_0} - 1$
    \item EstCostMoves($S,s,v$) := $d(v) - d(v, S)\frac{s}{\eta_0} + s - d(v, S)\frac{s}{\eta_0} - 1 = d(v) + s - 2d(v, S) \frac{s}{\eta_0} - 1$. 
\end{itemize}

We have that
\begin{enumerate}
    \item ExpCostStays($s,v$) := $\mathbb{E}_S[\text{EstCostStays($S,s,v$)}] = $ CostStays, and  
    \item ExpCostMoves($s,v$) := $\mathbb{E}_S[\text{EstCostMoves($S,s,v$)}] = $ CostMoves. 
\end{enumerate}

\end{lemma}

\hwcom{To use Chernoff bound, we need to make sure that everything is independent, to achieve this, we could make a uniform random multiset sample instead. }

\begin{lemma}
\label{lem:concentration}
Let $\eta_0 > 0$. Consider the setting of Lemma~\ref{lem:moves_estimate}, a vertex $v$ in
some good cluster $C(v)$, an arbitrary good cluster
$K$ of size $s > \eta_0^4$ and a random uniform sample $S$ of $K$ of size $\eta_0^4$.
Then, with probability at least  $1 - 2^{\eta_0^2}$ we have that the following
two inequalities hold:
\begin{enumerate}
    \item EstCostStays($S,s,v$) $\in$ ExpCostStays($s,v$) $\pm 1/\eta_0^2 (d^\adm(v) + |C(v)| + |K|)$, and 
\item EstCostMoves($S,s,v$) $\in$ ExpCostMoves($s,v)$ $\pm 1/\eta_0^2 (d^\adm(v) + |C(v)| + |K|)$.
\end{enumerate}
\end{lemma}
\begin{proof}
    \begin{align*}
        \rmCostStays(K,v) & = |C(v)| + d(v) - |C(v) \cap K| - 2d(v, C(v)) + 2d(v, C(v) \cap K) - 1 \\
        & \leq d^{adm}(v) + 1 + d(v) + 2|N| - 1 \\
        & \leq 4\epsilon^{-5}|N| + \epsilon^{-1}|N| + 2|N| \\
        & \leq 7\epsilon^{-5}|N| \\
        \rmCostMoves(K,v) & = d(v) + |K| - 2d(v, K) - 1 \\
        & \leq 2\epsilon^{-2}|N| + |N| \\
        & \leq 3\epsilon^{-2}|N|
    \end{align*}
    Chernoff bound.
\end{proof}

For a clustering $\calC$, we say that $\calC$ is \emph{clean} if for all  vertices $v$, we have that $\cost(\calC + \{v\}) \ge \cost(\calC)$. 


We now present the GenerateCluster procedure.
\begin{tcolorbox}[beforeafter skip=10pt]
    \textbf{GenerateCluster($\calC, r, K, S^1,\ldots,S^\eta, s^1,\ldots, s^\eta$)}
    \begin{itemize}[itemsep=0pt, topsep=4pt]
    \item Let $N_r$ be the set 
    of vertices of $u$ such that $(u,r)$ is admissible and that 
    are not in an atom.
    \begin{itemize}
    \item $S' \gets K$.
    \item Let $N_r^1, \ldots, N_r^{\eta}$ be an arbitrary partition of the
    vertices of $N_r$ into equal-size parts,
    \item For $i=1,\ldots,\eta$:
    \begin{itemize}
    \item For each vertex $v \in N_r^i$,
    \begin{itemize}[itemsep=0pt, topsep=4pt]
    \item Let $C(v)$ be the current cluster of $v$. 
    \item If EstCostStays($S^i,s_i,v$) $>$ EstCostMoves($S^i, s_i,v$) + $\eta^{-3} s_i$,\\ then $S' \gets S' \cup \{v\}$.
    \end{itemize}
    \end{itemize}
    
\end{itemize}   
    \item Return $S'$.
\end{itemize}
\end{tcolorbox}

We now aim at showing the following lemma.
\begin{lemma}
\label{lem:generate-cluster}
    Let $\eta < 1/\epsilon^{21}$ be a sufficiently large constant.
    Consider a clustering $\calC$ maintained by the local search algorithm and assume that there exists a good cluster $C$
    such that $\cost(\calC + C)  + 20\epsilon^7 \sum_{u \in C} d^{\adm}(u) \le \cost(\calC)$. Then
    there exists a collection of subsets $\mathcal{S} = S^1,\ldots,S^\eta$ each of at most $\eta^{5}$ vertices, and each collection of $\eta$ integers $\vec{s} = s^1,\ldots,s^\eta \in [|V|]$, 
    such that 
    the cluster $S'$ output by GenerateCluster($\calC, \mathcal{S}, \vec{s})$ satisfies
    \[\cost(\calC+S') < \cost(\calC)\]
\end{lemma}
\begin{proof}
Let $\calC = \{C_1,\ldots,C_k\}$. 
Let $C^* = \text{argmin}_{Q \subseteq N_r \cup K} \cost(\calC+Q)$, i.e.: the most
improving cluster of $N_r \cup K$. Let consider the iteration of the algorithm 
where both $K \subseteq C$ and $r \in C$ (note that $K$ could be empty so there
must be such an iteration).
Since $C$ is a good cluster containing $r$, and that each good cluster contains at most one atom, we have that $C \subseteq N_r \cup K$.
Thus, we have that $\cost(\calC+C^*) \le \cost(\calC+C) + 10\epsilon^{7} \sum_{u \in C} d^{\adm}(u) \le \cost(\calC)
- 10\epsilon^{7} \sum_{u \in C} d^{\adm}(u)$, so it is enough to show that GenerateCluster outputs a cluster of cost at most $\cost(\calC+C^*) + 5\epsilon^{7} \sum_{u \in C^*} d^{\adm}(u)$.
Let $s^* = |C^*|$. 
Note that since  we work with a good preclustered instance, we have that $|N_r|$ is proportional to the degree of $r$ and since $(u,r)$ is admissible for 
all $u \in N_r$, $d^{\adm}(u)$ is also proportional to $|N_r|$.  

Next, we argue that $s^* \ge \epsilon^{10} |N_r|$. The reason for this is 
$\calC$ is a clean clustering and so if $s^* < \epsilon^{10} |N_r|$, 
the cost improvement of creating $C^*$ is at most $(\epsilon^{10}|N_r|)^2$
and so $\cost(\calC+C^*) > \cost(\calC) - (\epsilon^{10}|N_r|)^2 
\ge \cost(\calC) - 10\eta^{-1} \sum_{v \in N_r} d^{\adm}(v)$. This combined 
with our choice of
$\eta$ and the fact that vertices in $N_r$ have degree proportional to $|N_r|$
would contradict our assumption on $\cost(\calC+ C)$.
We thus assume that $s^* \ge \epsilon^{10}|N_r|$ in the remaining.

We thus have the following property of $C^*$. Let $v$ be a vertex in $N_r$, 
if $v$ is not in an atom, then we have that by definition of $C^*$:
\begin{enumerate}
    \item if $v$ in $C^*$, then $\cost(\calC+(C^*\setminus \{v\})) \ge \cost(\calC+C^*)$; and
    \item if $v$ is not in $C^*$ then $\cost(\calC+(C^* \cup \{v\})) \ge 
    \cost(\calC+C^*)$.
\end{enumerate}

\todo{todo: change the indices from $i$ to $i-1$, etc.}
To analyze the algorithm, let $S'^{1},\ldots,S'^{\eta}$ be the set of elements in set $S'$ 
at the beginning of the $i$th iteration of the for loop.
We think of $S^i$ as a uniform sample of the cluster $C^*_i := S'^{i} \cup \bigcup_{j=i}^{\eta} (C^* \cap N_r^j)$ and $s_i$ as $|C^*_i|$.
We want to show the following claim.

\begin{claim}
\label{claim:invariant}
At iteration $i$, we have $\cost(\calC + C^*_i) \le \cost(\calC+C^*) + O(i \epsilon^{-2} \eta^{-2} \sum_{j=i}^j |N_r^j|)$, and $\forall j \ge i$, $\forall v \in N^j_r$ that is not in an atom, 
\begin{enumerate}
    \item if $v \in \bigcup_{j=i}^\eta (C^* \cap N^j_r)$, $\cost(\calC+(C_i^*\setminus \{v\})) \ge \cost(\calC+C_i^*)$; and
    \item if $v$ is not in $\bigcup_{j=i}^\eta (C^* \cap N^j_r)$ then $\cost(\calC+(C_i^* \cup \{v\})) \ge 
    \cost(\calC+C_i^*)$.
\end{enumerate}
\end{claim}

Assuming the claim is true, the lemma follows
by observing that (1) $S' = C^*_{\eta}$; and (2)
since $i$ ranges from $1$ to $\eta$, we have
that $\cost(\calC+S') \le \cost(\calC+C^*) +\epsilon^{-2} \eta^{-1}|N_r|^2$.

We conclude by observing 
that each vertex $u$ in $N_r$ is degree-similar to $r$ and so $d(u) \ge \epsilon d(r) \ge \epsilon^{4} |N_r|$ and 
so we have by our choice of $\eta$,
$\cost(\calC+S') \le \cost(\calC+C^*) + \eta^{-1}\sum_{u \in C^*} d^{\adm}(u)$, as desired. \todo{this last part needs to be tighten, the idea is that $\eta$
can be made as small as desired compared to $\epsilon$}

\begin{proof}[Proof of Claim~\ref{claim:invariant}]
We prove the claim by induction on $i$. By the above discussion, the claim
holds at $i = 1$.
We assume the claim holds for iteration $i$ and show that it holds for iteration $i+1$. We analyze the decisions made by our algorithm for the elements in $N_r^j$, 
namely whether they are added or not to $S'$. 

For a given vertex, recall that CostMoves and CostStays are respectively the cost
of $v \in N_r^i$ in the solution $\calC + (C^*_i \cup \{v\})$ and the cost of $v$ in the 
solution $\calC + (C^*_i \setminus \{v\})$. 
Since we work with a good preclustered instance, we note
that all the vertices considered below must have degree at most $|N_r|/\epsilon^4$ and at least $\epsilon^4 |N_r|$. 
Consider a vertex $v \not\in C^*_i$. then
we have that CostMoves $>$ CostStays. 

Then Lemma~\ref{lem:concentration}
implies that the probability that for $v \not\in C^*_i$, such that $(u,v)$ is
an admissible pair for all $u \in S$, the probability that EstCostMoves($s_i,v$) + $\eta^{-3} |N_r|$ $<$ EstCostStays($s_i,v$) is at most $\exp(-\eta^2)$. 
Thus, the expected number of vertices
$v \not\in C^*_i$ ending up in $S'$ is at most $|N_r^i| \exp(-\eta^2)$.
Since we work with a good preclustered instance, this is at most $\exp(-\eta^2) d^{\adm}(r) \epsilon^{-1} \le \eta^{-2} |N_r|$ for a sufficiently small $\eta$.
Since the degree of each vertex in the vertices $v \notin C^*_i$ that are added to $S'$ in this iteration of the GenerateCluster procedure is at most $|N_r|/\epsilon$, it 
follows that the overall cost incurred by this set is at most 
$O(\eta^{-2} |N_r|^2)$ for a sufficiently small $\eta$.


We now turn to the cost incurred by the vertices in $C^*_i$.
We distinguish two sets of nodes:
\begin{itemize}
    \item $v$ is a \emph{core} node if  $v \in C^*_i$ and that 
    CostMoves $+\eta^{-2}|N_r|$ $<$ CostStays.
    \item $v$ is a \emph{non-core} node if  $v \in C^*_i$ and that 
    CostMoves $+\eta^{-2}|N_r|$ $\ge$ CostStays.
\end{itemize}
 
Let us first consider the cost incurred by the core nodes. Again, 
Lemma~\ref{lem:concentration} implies that the probability of
a core node not joining $S'$ is at most $\exp(-\eta^2)$. It follows that the expected
number of core nodes not in $S'$ is at most $\eta^{-2} |N_r|$. The cost incurred
by this is thus at most $O(\eta^{-2}|N_r|^2)$.

We finally turn our attention to the cost incurred by the non-core nodes.
Consider any subset $L$ of non-core nodes and let's analyse the cost of 
leaving the vertices in $L$ in their original clusters in $\calC$. 
Since CostMoves $+\eta^{-2}|N_r|$ $\ge$ CostStays for each such vertex, the 
overall cost increase is thus at most $\eta^{-2}|N_r|^2$ plus the cost of moving or
not moving the vertices in the same $N^r_i$. Since $|N^r_i| \le \epsilon^{-1} |N_r|/ \eta$, 
we have that the cost increased for not adding these vertices is at most
$O(\epsilon^{-1} \eta^{-2}|N_r|^2)$.

Hence, let $Q^*_i := S'^{i+1} \cup \bigcup_{j=i+1}^{\eta} (C^* \cap N_r^j)$. 
As argued above $\cost(\calC+Q^*_i) \le \cost(\calC+C^*_i) + O(\epsilon^{-1} \eta^{-2}|N_r|^2)$.
We obtain $C^*_{i+1}$ by cleaning the vertices in $\bigcup_{j=i+1}^{\eta} N_r^j$: 
We let $C^*_{i+1} := S'^{i+1} \cup M$ where $M \subseteq  \bigcup_{j=i+1}^{\eta} N_r^j$ such that all the vertices in $M$ are clean
with respect to $\calC+C^*_{i+1}$ and $C^*_{i+1}$ is such that 
$\calC+C^*_{i+1}$ is of minimum cost. We thus have that 
$\cost(\calC+C^*_{i+1}) \le \cost(\calC+Q^*_i) \le cost(\calC+C^*_i) + O(\epsilon^{-1} \eta^{-2}|N_r|^2)$ and the vertices satisfies bullet (1) 
and (2) of the Claim. 
It follows that the cost of moving from set $C^*_i$ to $C^*_{i+1}$ is only $\epsilon^{-1} \eta^{-2} |N_r|$ as desired. The induction hypothesis is thus
satisfied and this conclude the proof of the claim.
\end{proof}
\end{proof}%






In the rest of the draft, we only consider a fixed good preclustered instance
$(\calK, E_{\adm})$. 
Given a clustering $\calC = \{C_1,\ldots,C_k\}$, and a set $C'$ we denote
by $\calC + C'$ the clustering defined by 
$\{C_1 \setminus C', \ldots, C_k \setminus C', C'\}$.


{\color{magenta}



\begin{theorem}
Also, let $\gamma < \epsilon^7/2 $ be sufficiently small relative to $\epsilon$. Consider a clustering $\calC$ and assume that there is no good 
cluster $C^*$
such that the cost of 
\begin{equation}\label{eq:improve+}
\cost(\calC + C^*)  + \gamma \sum_{u \in C^*} d^{adm}(u) \le \cost(\calC).    
\end{equation}
Then $\calC$ almost locally optimal
in our local search sense, up to an additive term of $\epsilon \cost(\opt)$.
\end{theorem}
\begin{proof}
    This is a quite direct consequence
    of Theorem \ref{thm:preprocessed-wrapper} together with our general
    understanding of the use of local search.
\end{proof}

Thus, to get for our local search to work, it suffices to find
an "improving" cluster $C$ with 
    \[\cost(\calC+C) < \cost(\calC)\]
if there exists a good cluster $C^*$
satisfying \req{eq:improve+}. Below
we assume that such a cluster exists, and then, by reference to the unknown $C^*$, we will derive an improving cluster $C$. First, if $C^*$ is an atom, then we get it directly from
the pre-clustering, so we can assume that $C^*$ is not just an atom.

First we give an abstract deterministic algorithm, that may seem silly, but which conveys the basic accounting atoms.

First we guess an $r\in C^*$ and moreover if $C^*$ contains an atom $K$, let $r \in K$.
Let $N_r$ be the set of vertices $u$ such that 
$(r,u)$ is admissible. Then $N_r\supseteq C^*$. 
\mikcom{PROBLEM? I think the current analysis tries to exploit $|N_r|=O(|C^*|)$ and $\sum_{u \in N_r\setminus V_{\calK}} d(u)=O(\sum_{u \in C^*} d(u))$, but we could still have $|N_r\setminus V_{\calK}|\gg |C^*\setminus V_{\calK}|$.\\
SOLUTION?? If we look to approximate a a good cluster $C^*$ containing an atom $K$, then instead of using $N_r$,
we can use $N_K$ consisting of $K$ and all
vertices that are admissible neighbors of all vertices in $K$. Now I think
we can prove $\sum_{u \in N_K\setminus K} d(u)=O(\sum_{u \in C^*} d^{adm}(u))$.\\}
\mikcom{
META PROBLEM FOR ME: It is not sufficiently clear to me what values we are trying amortize our estimate errors over. I would have liked it to be bounded as in \req{eq:improve+}
\vcacom{The fix is correct, 
we would like to amortize over the admissible edges of $r$. The idea is
that we make no mistake for the edges where both endpoint are in the atom $K$ of $C^*$ since it gets included directly. We make a number of mistakes proportional to for the admissible degrees of the 
clusters elements.}


If $C^*$ has an atom $K$, define $N:=N_K$ , and $D:=N_K\setminus K$; otherwise,
for some $r\in C^*$, let $N:=N_r$ and $D:=N_r\setminus\{r\}$. 
\begin{lemma} 
    $|D|\cdot |N|=\epsilon^{-4}(\sum_{u \in C^*} d^{adm}(u))$.
\end{lemma}
\begin{proof}
The new case in the proof is when
$|K|\geq|N_K|/2$. In this case, since $K\subseteq C^*$, we
exploit that $\sum_{u\in K}d^{adm}(u)\geq |D|\cdot|K|$. 
\end{proof}
}
I think we are now ready to introduce the approach with sampling. That we
start from $C=C^*$, and then we
ask for each vertex $v\in D$ if
it is better for $\cal C+C$ if we
put $v$ in $C$ or not, updating $C$ accordingly. If we
knew the exact answer and there were no ties, then by local optimality of $C^*$, we would not make any changes
to $C$, but the algorithm is as
described is only an abstraction
as we do not know $C^*$. However,
we will assume some lucky samples 
that allow us to approximate whether or not the vertices should be in $C$,
and we will amortize the errors over 
$|D|\cdot |N|$.
}

For a clustering $\calC$, and a vertex $v$ we say that $v$ is \emph{clean} with respect to $\calC$ if $\cost(\calC + \{v\}) \ge \cost(\calC)$. When $\calC$ is clear from the context we simply say that $v$ is clean. We say that $\calC$ is \emph{clean} if all vertices $v$ are clean with respect to $\calC$.

We will consider the following local search algorithm, with parameter $\eta$.
\begin{tcolorbox}[beforeafter skip=10pt]
    \textbf{Local Search with good clusters($\eta$)}
    \begin{itemize}[itemsep=0pt, topsep=4pt]
    \item Compute an atomic pre-clustering using the Precluster algorithm.
        \item $\calC \gets $ Arbitrary clean good clustering of the preclustered instance (e.g.: the clustering returned by \cite{CLLN23+}).
        \item Do
        \begin{itemize}[itemsep=0pt, topsep=4pt]
        \item For each vertex $r$, each $K \in \calK \cup \{\emptyset\}$, for each collection of  $\eta$ (not necessarily disjoint) subsets $\mathcal{S} = S^1,\ldots,S^\eta$ each of at most $\eta^{5}$ vertices that are not in an atom, and each collection of $\eta$ integers $\vec{s} = s^1,\ldots,s^\eta \in [|V|]$, \\
        $\calC(\mathcal{S},\vec{s}) \gets  \calC + $ GenerateCluster($\calC, r, K, S^1,\ldots,S^\eta, s^1,\ldots,s^\eta$).
        \item Let $\mathcal{S}^*, \vec{s}^*$ be the pair such that the cost of $\calC(\mathcal{S}^*, \vec{s}^*)$ is minimized.
        \item If the cost of $\calC(\mathcal{S}^*, \vec{s}^*)$ is less than the cost of $\calC$:
        \begin{itemize}
            \item has\_improved $\gets$ true;
            \item $\calC \gets \calC(\mathcal{S}^*, \vec{s}^*)$;
            \item Cleaning step: While there exists a vertex $v$ such that $v$ is not adjacent to at least $1/2$ of
            the vertices in its cluster in $\calC$, make $v$ a singleton. This
            ensures that $\calC$ is clean.
        \end{itemize}
        \item Else has\_improved $\gets$ false
        \end{itemize}
        \item While has\_improved
        \item Output $\calC$
    \end{itemize}
\end{tcolorbox}

\begin{fact}
\label{fact:clean}
At the beginning of each iteration of the Do-While loop, the clustering
$\calC$ is clean.
\end{fact}





\vcacom{The main idea behind generate good cluster is to build it in $\eta$ steps. Each step adds at most roughly a $1/\eta$ fraction of the vertices. this ensures that the sampling is correct / not impacted by the decision made for the vertices considered during the same step. in other words, the assignments of the vertices at a given step are independent of each other}
\begin{definition}
Consider a clustering $\calC$ of the graph and
let $v$ be a vertex, $C(v)$ its cluster and $K$
an arbitrary set of vertices.
We consider the clustering $\calC+K$

We define CostStays($K,v$) to be the number of edges $(u,v)$
that are violated in $\calC+(K\setminus \{v\})$ and CostMoves($K,v$) to
be the number of edges $(u,v)$ that are violated
in $\calC+(K\cup\{v\})$.

We have
\begin{enumerate}
    \item $\rmCostStays(K,v) = d(v) - d(v, C(v)) + d(v, C(v) \cap K) + |C(v)| - |C(v) \cap K| - d(v, C(v)) + d(v, C(v) \cap K) - 1$ where $d(v) - d(v, C(v)) + d(v, C(v) \cap K)$ is the contribution of the $+$ edges and $|C(v)| - |C(v) \cap K| - d(v, C(v)) + d(v, C(v) \cap K) - 1$ the contribution of the $-$ edges.
    
    Which is 
    equal to $|C(v)| + d(v) - |C(v) \cap K| - 2d(v, C(v)) + 2d(v, C(v) \cap K) - 1$.
    \item $\rmCostMoves(K,v) = d(v) - d(v, K) + |K| - d(v,K) - 1 = d(v) + |K| - 2d(v, K) - 1$. 
\end{enumerate}
\end{definition}

\begin{lemma}
\label{lem:moves_estimate}
Let $\eta_0 > 1$.
    Consider a clustering $\calC$ of the graph and
let $v$ be a vertex, $C(v)$ its cluster and $K$
an arbitrary set of vertices of size $s > \eta_0$.
 Furthermore, let $S$ be a uniform sample of $K$ of size $\eta_0$.
Consider the clustering $\calC+K$
We define the following random variables
\begin{itemize}
    \item EstCostStays($S,s,v$) := $|C(v)| + d(v) - |C(v) \cap S| \frac{s}{\eta_0} - 2d(v, C(v)) + 2d(v, C(v) \cap S) \frac{s}{\eta_0} - 1$
    \item EstCostMoves($S,s,v$) := $d(v) - d(v, S)\frac{s}{\eta_0} + s - d(v, S)\frac{s}{\eta_0} - 1 = d(v) + s - 2d(v, S) \frac{s}{\eta_0} - 1$. 
\end{itemize}

We have that
\begin{enumerate}
    \item ExpCostStays($s,v$) := $\mathbb{E}_S[\text{EstCostStays($S,s,v$)}] = $ CostStays, and  
    \item ExpCostMoves($s,v$) := $\mathbb{E}_S[\text{EstCostMoves($S,s,v$)}] = $ CostMoves. 
\end{enumerate}

\end{lemma}

\hwcom{To use Chernoff bound, we need to make sure that everything is independent, to achieve this, we could make a uniform random multiset sample instead. }

\begin{lemma}
\label{lem:concentration}
Let $\eta_0 > 0$. Consider the setting of Lemma~\ref{lem:moves_estimate}, a vertex $v$ in
some good cluster $C(v)$, an arbitrary good cluster
$K$ of size $s > \eta_0^4$ and a random uniform sample $S$ of $K$ of size $\eta_0^4$.
Then, with probability at least  $1 - 2^{\eta_0^2}$ we have that the following
two inequalities hold:
\begin{enumerate}
    \item EstCostStays($S,s,v$) $\in$ ExpCostStays($s,v$) $\pm 1/\eta_0^2 (d^\adm(v) + |C(v)| + |K|)$, and 
\item EstCostMoves($S,s,v$) $\in$ ExpCostMoves($s,v)$ $\pm 1/\eta_0^2 (d^\adm(v) + |C(v)| + |K|)$.
\end{enumerate}
\end{lemma}
\begin{proof}
    \begin{align*}
        \rmCostStays(K,v) & = |C(v)| + d(v) - |C(v) \cap K| - 2d(v, C(v)) + 2d(v, C(v) \cap K) - 1 \\
        & \leq d^{adm}(v) + 1 + d(v) + 2|N| - 1 \\
        & \leq 4\epsilon^{-5}|N| + \epsilon^{-1}|N| + 2|N| \\
        & \leq 7\epsilon^{-5}|N| \\
        \rmCostMoves(K,v) & = d(v) + |K| - 2d(v, K) - 1 \\
        & \leq 2\epsilon^{-2}|N| + |N| \\
        & \leq 3\epsilon^{-2}|N|
    \end{align*}
    Chernoff bound.
\end{proof}

For a clustering $\calC$, we say that $\calC$ is \emph{clean} if for all  vertices $v$, we have that $\cost(\calC + \{v\}) \ge \cost(\calC)$. 


We now present the GenerateCluster procedure.
\begin{tcolorbox}[beforeafter skip=10pt]
    \textbf{GenerateCluster($\calC, r, K, S^1,\ldots,S^\eta, s^1,\ldots, s^\eta$)}
    \begin{itemize}[itemsep=0pt, topsep=4pt]
    \item Let $N_r$ be the set 
    of vertices of $u$ such that $(u,r)$ is admissible and that 
    are not in an atom.
    \begin{itemize}
    \item $S' \gets K$.
    \item Let $N_r^1, \ldots, N_r^{\eta}$ be an arbitrary partition of the
    vertices of $N_r$ into equal-size parts,
    \item For $i=1,\ldots,\eta$:
    \begin{itemize}
    \item For each vertex $v \in N_r^i$,
    \begin{itemize}[itemsep=0pt, topsep=4pt]
    \item Let $C(v)$ be the current cluster of $v$. 
    \item If EstCostStays($S^i,s_i,v$) $>$ EstCostMoves($S^i, s_i,v$) + $\eta^{-3} s_i$,\\ then $S' \gets S' \cup \{v\}$.
    \end{itemize}
    \end{itemize}
    
\end{itemize}   
    \item Return $S'$.
\end{itemize}
\end{tcolorbox}

We now aim at showing the following lemma.
\begin{lemma}
\label{lem:generate-cluster}
    Let $\eta < 1/\epsilon^{21}$ be a sufficiently large constant.
    Consider a clustering $\calC$ maintained by the local search algorithm and assume that there exists a good cluster $C$
    such that $\cost(\calC + C)  + 20\epsilon^7 \sum_{u \in C} d^{\adm}(u) \le \cost(\calC)$. Then
    there exists a collection of subsets $\mathcal{S} = S^1,\ldots,S^\eta$ each of at most $\eta^{5}$ vertices, and each collection of $\eta$ integers $\vec{s} = s^1,\ldots,s^\eta \in [|V|]$, 
    such that 
    the cluster $S'$ output by GenerateCluster($\calC, \mathcal{S}, \vec{s})$ satisfies
    \[\cost(\calC+S') < \cost(\calC)\]
\end{lemma}
\begin{proof}
Let $\calC = \{C_1,\ldots,C_k\}$. 
Let $C^* = \text{argmin}_{Q \subseteq N_r \cup K} \cost(\calC+Q)$, i.e.: the most
improving cluster of $N_r \cup K$. Let consider the iteration of the algorithm 
where both $K \subseteq C$ and $r \in C$ (note that $K$ could be empty so there
must be such an iteration).
Since $C$ is a good cluster containing $r$, and that each good cluster contains at most one atom, we have that $C \subseteq N_r \cup K$.
Thus, we have that $\cost(\calC+C^*) \le \cost(\calC+C) + 10\epsilon^{7} \sum_{u \in C} d^{\adm}(u) \le \cost(\calC)
- 10\epsilon^{7} \sum_{u \in C} d^{\adm}(u)$, so it is enough to show that GenerateCluster outputs a cluster of cost at most $\cost(\calC+C^*) + 5\epsilon^{7} \sum_{u \in C^*} d^{\adm}(u)$.
Let $s^* = |C^*|$. 
Note that since  we work with a good preclustered instance, we have that $|N_r|$ is proportional to the degree of $r$ and since $(u,r)$ is admissible for 
all $u \in N_r$, $d^{\adm}(u)$ is also proportional to $|N_r|$.  

Next, we argue that $s^* \ge \epsilon^{10} |N_r|$. The reason for this is 
$\calC$ is a clean clustering and so if $s^* < \epsilon^{10} |N_r|$, 
the cost improvement of creating $C^*$ is at most $(\epsilon^{10}|N_r|)^2$
and so $\cost(\calC+C^*) > \cost(\calC) - (\epsilon^{10}|N_r|)^2 
\ge \cost(\calC) - 10\eta^{-1} \sum_{v \in N_r} d^{\adm}(v)$. This combined 
with our choice of
$\eta$ and the fact that vertices in $N_r$ have degree proportional to $|N_r|$
would contradict our assumption on $\cost(\calC+ C)$.
We thus assume that $s^* \ge \epsilon^{10}|N_r|$ in the remaining.

We thus have the following property of $C^*$. Let $v$ be a vertex in $N_r$, 
if $v$ is not in an atom, then we have that by definition of $C^*$:
\begin{enumerate}
    \item if $v$ in $C^*$, then $\cost(\calC+(C^*\setminus \{v\})) \ge \cost(\calC+C^*)$; and
    \item if $v$ is not in $C^*$ then $\cost(\calC+(C^* \cup \{v\})) \ge 
    \cost(\calC+C^*)$.
\end{enumerate}

\todo{todo: change the indices from $i$ to $i-1$, etc.}
To analyze the algorithm, let $S'^{1},\ldots,S'^{\eta}$ be the set of elements in set $S'$ 
at the beginning of the $i$th iteration of the for loop.
We think of $S^i$ as a uniform sample of the cluster $C^*_i := S'^{i} \cup \bigcup_{j=i}^{\eta} (C^* \cap N_r^j)$ and $s_i$ as $|C^*_i|$.
We want to show the following claim.

\begin{claim}
\label{claim:invariant}
At iteration $i$, we have $\cost(\calC + C^*_i) \le \cost(\calC+C^*) + O(i \epsilon^{-2} \eta^{-2} \sum_{j=i}^j |N_r^j|)$, and $\forall j \ge i$, $\forall v \in N^j_r$ that is not in an atom, 
\begin{enumerate}
    \item if $v \in \bigcup_{j=i}^\eta (C^* \cap N^j_r)$, $\cost(\calC+(C_i^*\setminus \{v\})) \ge \cost(\calC+C_i^*)$; and
    \item if $v$ is not in $\bigcup_{j=i}^\eta (C^* \cap N^j_r)$ then $\cost(\calC+(C_i^* \cup \{v\})) \ge 
    \cost(\calC+C_i^*)$.
\end{enumerate}
\end{claim}

Assuming the claim is true, the lemma follows
by observing that (1) $S' = C^*_{\eta}$; and (2)
since $i$ ranges from $1$ to $\eta$, we have
that $\cost(\calC+S') \le \cost(\calC+C^*) +\epsilon^{-2} \eta^{-1}|N_r|^2$.

We conclude by observing 
that each vertex $u$ in $N_r$ is degree-similar to $r$ and so $d(u) \ge \epsilon d(r) \ge \epsilon^{4} |N_r|$ and 
so we have by our choice of $\eta$,
$\cost(\calC+S') \le \cost(\calC+C^*) + \eta^{-1}\sum_{u \in C^*} d^{\adm}(u)$, as desired. \todo{this last part needs to be tighten, the idea is that $\eta$
can be made as small as desired compared to $\epsilon$}

\begin{proof}[Proof of Claim~\ref{claim:invariant}]
We prove the claim by induction on $i$. By the above discussion, the claim
holds at $i = 1$.
We assume the claim holds for iteration $i$ and show that it holds for iteration $i+1$. We analyze the decisions made by our algorithm for the elements in $N_r^j$, 
namely whether they are added or not to $S'$. 

For a given vertex, recall that CostMoves and CostStays are respectively the cost
of $v \in N_r^i$ in the solution $\calC + (C^*_i \cup \{v\})$ and the cost of $v$ in the 
solution $\calC + (C^*_i \setminus \{v\})$. 
Since we work with a good preclustered instance, we note
that all the vertices considered below must have degree at most $|N_r|/\epsilon^4$ and at least $\epsilon^4 |N_r|$. 
Consider a vertex $v \not\in C^*_i$. then
we have that CostMoves $>$ CostStays. 

Then Lemma~\ref{lem:concentration}
implies that the probability that for $v \not\in C^*_i$, such that $(u,v)$ is
an admissible pair for all $u \in S$, the probability that EstCostMoves($s_i,v$) + $\eta^{-3} |N_r|$ $<$ EstCostStays($s_i,v$) is at most $\exp(-\eta^2)$. 
Thus, the expected number of vertices
$v \not\in C^*_i$ ending up in $S'$ is at most $|N_r^i| \exp(-\eta^2)$.
Since we work with a good preclustered instance, this is at most $\exp(-\eta^2) d^{\adm}(r) \epsilon^{-1} \le \eta^{-2} |N_r|$ for a sufficiently small $\eta$.
Since the degree of each vertex in the vertices $v \notin C^*_i$ that are added to $S'$ in this iteration of the GenerateCluster procedure is at most $|N_r|/\epsilon$, it 
follows that the overall cost incurred by this set is at most 
$O(\eta^{-2} |N_r|^2)$ for a sufficiently small $\eta$.


We now turn to the cost incurred by the vertices in $C^*_i$.
We distinguish two sets of nodes:
\begin{itemize}
    \item $v$ is a \emph{core} node if  $v \in C^*_i$ and that 
    CostMoves $+\eta^{-2}|N_r|$ $<$ CostStays.
    \item $v$ is a \emph{non-core} node if  $v \in C^*_i$ and that 
    CostMoves $+\eta^{-2}|N_r|$ $\ge$ CostStays.
\end{itemize}
 
Let us first consider the cost incurred by the core nodes. Again, 
Lemma~\ref{lem:concentration} implies that the probability of
a core node not joining $S'$ is at most $\exp(-\eta^2)$. It follows that the expected
number of core nodes not in $S'$ is at most $\eta^{-2} |N_r|$. The cost incurred
by this is thus at most $O(\eta^{-2}|N_r|^2)$.

We finally turn our attention to the cost incurred by the non-core nodes.
Consider any subset $L$ of non-core nodes and let's analyse the cost of 
leaving the vertices in $L$ in their original clusters in $\calC$. 
Since CostMoves $+\eta^{-2}|N_r|$ $\ge$ CostStays for each such vertex, the 
overall cost increase is thus at most $\eta^{-2}|N_r|^2$ plus the cost of moving or
not moving the vertices in the same $N^r_i$. Since $|N^r_i| \le \epsilon^{-1} |N_r|/ \eta$, 
we have that the cost increased for not adding these vertices is at most
$O(\epsilon^{-1} \eta^{-2}|N_r|^2)$.

Hence, let $Q^*_i := S'^{i+1} \cup \bigcup_{j=i+1}^{\eta} (C^* \cap N_r^j)$. 
As argued above $\cost(\calC+Q^*_i) \le \cost(\calC+C^*_i) + O(\epsilon^{-1} \eta^{-2}|N_r|^2)$.
We obtain $C^*_{i+1}$ by cleaning the vertices in $\bigcup_{j=i+1}^{\eta} N_r^j$: 
We let $C^*_{i+1} := S'^{i+1} \cup M$ where $M \subseteq  \bigcup_{j=i+1}^{\eta} N_r^j$ such that all the vertices in $M$ are clean
with respect to $\calC+C^*_{i+1}$ and $C^*_{i+1}$ is such that 
$\calC+C^*_{i+1}$ is of minimum cost. We thus have that 
$\cost(\calC+C^*_{i+1}) \le \cost(\calC+Q^*_i) \le cost(\calC+C^*_i) + O(\epsilon^{-1} \eta^{-2}|N_r|^2)$ and the vertices satisfies bullet (1) 
and (2) of the Claim. 
It follows that the cost of moving from set $C^*_i$ to $C^*_{i+1}$ is only $\epsilon^{-1} \eta^{-2} |N_r|$ as desired. The induction hypothesis is thus
satisfied and this conclude the proof of the claim.
\end{proof}
\end{proof}


==> polytime-local-search-old4.1.tex <==
\begin{tcolorbox}[beforeafter skip=10pt]
    \textbf{GenerateCluster($\calC, r, K, S^1,\ldots,S^\eta, s^1,\ldots, s^\eta$)}    
\begin{itemize}[itemsep=0pt, topsep=4pt]
    \item $S' \gets K \cup \{r\}$.
    \item Let $D_r^1, \ldots, D_r^{\eta}$ be an arbitrary partition of the
    vertices of $D(r)$ into equal-size parts,
    \item For $i=1,\ldots,\eta$:
    \begin{itemize}
    \item For each vertex $v \in D_r^i$,
    \begin{itemize}[itemsep=0pt, topsep=4pt]
    \item Let $C(v)$ be the current cluster of $v$. 
    \item If EstCostStays($S^i,s_i,v$) $>$ EstCostMoves($S^i, s_i,v$) + $6\eta^{-1} W|N(r)|$,\\ then $S' \gets S' \cup \{v\}$.
    \end{itemize}
    \end{itemize}
    \item Return $S'$.
\end{itemize}
\end{tcolorbox}


\begin{lemma} 
\label{lem:D-times-N}
    For any vertex $v$ and any good cluster $C$ containing $v$, 
    \[
        \frac{1}{144}\epsilon^{8}|D(v)|\cdot |N(v)| \le \sum_{u \in C} d^{adm}(u) ~.
    \]
\end{lemma}

\begin{proof}
    Since $C$ is a good cluster, we have $|C| \geq \epsilon d(v) \geq \frac{1}{6}\epsilon^4 |N(v)|$. 
    If $v$ doesn't belong to any atom, then $|D(v)| = |N(v)| - 1$ and for every $u, v \in C$, they are admissible. Therefore
    \[
        \sum_{u \in C}d^{\adm}(u) \geq |C|(|C| - 1) \geq \frac{1}{2}|C|^2 \geq \frac{1}{72}\epsilon^8|N(v)|^2 \geq \frac{1}{72}\epsilon^8|D(v)|\cdot|N(v)| ~.
    \]

    Now suppose $v$ belongs to an atom $K$. If $|K| \geq \alpha |N(v)|$, then 
    \[
        \sum_{u \in C}d^{\adm}(u) \geq \sum_{u \in K}d^{\adm}(u) \geq \alpha|N(v)|\cdot |D(v)| ~.
    \]
    If $|K| \leq \alpha |N(v)|$, then 
    \[
        \sum_{u \in C}d^{\adm}(u) \geq \sum_{u \in C \setminus K}d^{\adm}(u) \geq (|C| - |K|)(|C| - 1) \geq \frac{1}{2}|C|(|C| - |K|) \geq \frac{1}{12}\epsilon^4(\frac{1}{6}\epsilon^4 - \alpha)|N(v)|^2 ~.
    \]
    Let $\alpha = \frac{1}{12}\epsilon^8$, the lemma always holds. 
\end{proof}

\mpcom{I added quantification over $r$ and $K$. Should we also take care of the case $K = \emptyset$?}
\hwcom{The new algorithm description says better. So in the algorithm, we just enumerate an vertex $r$ over $V$. If $v$ is contained in an atom, then $K$ is the atom; otherwise $K = \emptyset$. }
\begin{lemma}
\label{lem:generate-cluster}
Let $0 < \gamma < \epsilon^{13}/4$ and let $\eta > 1152 \epsilon^{-8} \gamma^{-1}$ be a sufficiently large constant so that
$2^{-\eta^2/2} < 0.01\eta^{-2} \epsilon^6$.

Consider a clustering $\calC$ maintained by the local search algorithm and assume that there exists a vertex $r$, and a good cluster $C$ with $K(r) \subseteq C \subseteq N(r)$
such that $|C| > 1$ and 
\[
    \cost(\calC + C)  + \gamma \sum_{u \in C} d^{\adm}(u) \le \cost(\calC) ~.
\]
Then there exists a collection of sets $C^*_1, \dots, C^*_{\eta}$, such that $K(r) \subseteq C^*_i \subseteq N(r)$, $|C^*_i| \geq \frac{1}{14400} \gamma\epsilon^{14} |N(r)|$. Let $\mathcal{S} = S^1,\ldots,S^\eta$, where $S^i$ is an uniform sample of $C^*_i$ of size $\eta^5$, let $\vec{s} = s^1 = |C^*_1|,\ldots, s^\eta = |C^*_\eta| \in [|V|]$. Then with probability at least $1 - 2\eta\exp(-\eta)$, 
the cluster $S'$ output by GenerateCluster($\calC, \mathcal{S}, \vec{s})$ satisfies
\[\cost(\calC+S') \leq \cost(\calC + C) +  \frac{\gamma}{2}\sum_{u \in C}d^{\adm}(u)\]
\end{lemma}
\begin{proof}
Fix $K$ and $r$ as in the lemma statement and let 
\[ C^* = \text{argmin}_{K(r) \subseteq Q \subseteq N(r)} \cost(\calC+Q).\]
That is,  $C^\ast$ is the most
improving cluster in $N(r)$ containing $K(r)$. 
Consider the iteration of the algorithm when we hit $r$. 
Since $C$ is a good cluster containing $r$, and that each good cluster contains at most one atom, we have that $C \subseteq N(r)$. 
Thus, we have that $\cost(\calC+C^*) \le \cost(\calC+C) \le \cost(\calC)
- \gamma \sum_{u \in C} d^{\adm}(u)$, so it is enough to show that GenerateCluster outputs a cluster of cost at most $\cost(\calC+C^*) + \frac{\gamma}{2} \sum_{u \in C} d^{\adm}(u)$.


Since $C$ is a good cluster containing $K \cup \{r\}$, $|C| \geq \epsilon d(v)$ for all $v \in K \cup \{r\}$, therefore $|N(r)| \geq |C| \geq \epsilon d(v)$. 

\begin{claim}
    \label{claim:degree}
    For any $v \in N(r)$,
    \[ d(v) \leq 2\epsilon^{-2}|N(r)|\quad\mathrm{and}\quad
       d^{\adm}(v) \leq 4\epsilon^{-5}|N(r)|.\]
\end{claim}
\begin{proof}
We first prove the first inequality.
    If $r, v$ are in the same cluster $K$, then $N(r) \geq \epsilon d(v)$; otherwise, $v$ is admissible to $r$, therefore $d(v) \leq 2\epsilon^{-1}d(r)$. 
    Furthermore, as $C$ is a good cluster contained in
    $N(r)$, we have $|N(r)| \geq |C| \geq \epsilon d(r)$.
    Hence, $d(v) \leq 2\epsilon^{-2} |N(r)|$, as desired.

The second inequality follows from the first 
and the condition $d^{\adm}(v) \leq 2\epsilon^{-3}d(v)$.
\end{proof}

Let $s^* = |C^*|$. Next, we will give a lowerbound on $s^*$. 
To this end, we show a quite brute-force estimate that adding one new cluster to a clustering scheme cannot improve the cost
by too much --- only roughly linear to the size of the new cluster.

\begin{claim}\label{claim:single-improvement}
    Let $\calC = \{C_1, \dots, C_k\}$ be a clustering maintained by the local search algorithm, $C \subseteq |N(r)|$ is any cluster, then
    \[ \cost(\calC) - 25\epsilon^{-6}|C|\cdot |N(r)| \leq \cost(\calC + C). \]
\end{claim}
\begin{proof}
    We split the cost improvement into two terms. The first term is the improvement on $E^+$, which is at most $\frac{1}{2}|C|(|C| - 1) \leq |C| \cdot |N(r)|$. 
    The second term is the improvement on $E^-$, which is at most the maximum amount of cost we pay before. 
    Let $v$ be an arbitrary vertex in $C$, $C_i$ be the cluster in $\calC$ containing $v$, the minus cost we pay in $\calC$ at $v$ is at most $|C_i| - 1$. 
    According to lemma~\ref{lem:bounded-minus-cost}, $|C_i| \leq 12\epsilon^{-4}d(v)$. 
    According to claim~\ref{claim:degree}, for all $v \in N(r)$, $d(v) \leq 2\epsilon^{-1}d(r) \leq 2\epsilon^{-2}|N(r)|$. 
    So we have the total improvement on $E^-$ is at most $12\epsilon^{-4}|C| \cdot (2\epsilon^{-2}|N(r)|) = 24\epsilon^{-6}|C|\cdot |N(r)|$. 
    Together with the improvement in the first part, the whole claim holds. 
\end{proof}

Observe that by lemma~\ref{lem:D-times-N}, we have
\[ \sum_{u \in C} d^{\adm}(u) \geq \frac{1}{144}\epsilon^8|D(r)|\cdot|N(r)|.\]
Hence, 
\[\cost(\calC + C^*) \leq \cost(\calC) - \gamma \sum_{u \in C}d^{\adm}(u) \leq \cost(\calC) - \frac{1}{144}\gamma \epsilon^8|D(r)|\cdot|N(r)|.\]
Together with Claim~\ref{claim:single-improvement} for $C^*$,
it follows that
\begin{equation}\label{eq:s-ast-bound}
s^* = |C^*| \geq \frac{1}{3600} \gamma \epsilon^{14} |D(r)|.
\end{equation}

Let $v$ be a vertex in $D(r)$, according to the optimality of $C^*$, we have
\begin{enumerate}
    \item if $v$ in $C^*$, then $\cost(\calC+(C^*\setminus \{v\})) \ge \cost(\calC+C^*)$; and
    \item if $v$ is not in $C^*$ then $\cost(\calC+(C^* \cup \{v\})) \ge 
    \cost(\calC+C^*)$.
\end{enumerate}

To analyze the algorithm, let $S'^{1},\ldots,S'^{\eta}$ be the set of elements in set $S'$ 
at the beginning of the $i$th iteration of the for loop. 
We define 
\[ C^*_i = S'^{i} \cup \mathrm{argmin} \left\{ \cost(\calC + (S'^{i} \cup T))~\Big|~T \subseteq \bigcup_{j = i}^{\eta}D_r^i\right\}.\]
Let $S^i$ be a uniform sample of the cluster $C^*_i$ and $s_i = |C^*_i|$. 
We want to show the following claim.

\begin{claim}
\label{claim:invariant}
With probability at least $1 - 2\exp(-\eta)$,
\[ \cost(\calC + C^*_{i+1}) - \cost(\calC+C^*_i) \le 4 \eta^{-2} |D(r)| \cdot |N(r)|. \] 
\end{claim}

Assuming the claim is true, with probability at least $1 - 2\eta \exp(-\eta)$, this claim holds for all $i = 1, \dots, \eta$. 
Then the lemma follows by observing that $S' = C^*_{\eta+1}$ and $C^*_1 = C^*$. 
By telescoping and Lemma~\ref{lem:D-times-N}, we have
\begin{align*}
    \cost(\calC+S') & = \cost(\calC+C^*) + \sum_{i = 1}^{\eta}(\cost(\calC + C^*_{i+1}) - \cost(\calC + C^*_i)) \\
    & \le \cost(\calC + C^*) + 4 \eta^{-1} \cdot |D(r)|\cdot |N(r)| \\ 
    & \le \cost(\calC+C^*) + 4 \eta^{-1} \cdot 144 \epsilon^{-8} \sum_{u \in C}d^{\adm}(u) \\
    & \le \cost(\calC + C)  + \frac{\gamma}{2} \sum_{u \in C}d^{\adm}(u)
\end{align*}
The last inequality follows from the assumption $\eta > 1152 \epsilon^{-8}\gamma^{-1}$. 

The only thing we miss is to show that $|C^*_i| \geq \frac{1}{14400} \gamma\epsilon^{14} |N(r)|$. By telescoping, we have
\begin{align*}
    \cost(\calC + C^*_i) & = \cost(\calC + C^*) + \sum_{j = 1}^{i - 1}(\cost(\calC + C^*_{j+1}) - \cost(\calC + C^*_i)) \\
    & \leq \cost(\calC + C^*) + (i - 1) \cdot 4\eta^{-2}|D(r)|\cdot|N(r)| \\
    & \leq \cost(\calC) - \frac{1}{144}\gamma\epsilon^{8}|D(r)|\cdot|N(r)| + 4\eta^{-1}|D(r)|\cdot|N(r)| \\
    & \leq \cost(\calC) - \frac{1}{288}\gamma \epsilon^{8}|D(r)|\cdot|N(r)|
\end{align*}
The last inequality holds from the assumption $\eta > 1152\epsilon^{-8}\gamma^{-1}$ and $\epsilon < 1$. 
Together with claim~\ref{claim:single-improvement} for $C^*_i$, it follows that
\[
    |C^*_i| \geq \frac{1}{7200} \gamma\epsilon^{14} |D(r)| ~.
\]
Since $K(r) \subseteq C^*_i$ and $|N(r)| = |D(r)| + |K(r)|$, we have
\begin{equation}\label{eq:size-of-sets-lowerbound}
    |C^*_i| \geq \frac{1}{14400} \gamma\epsilon^{14} |N(r)| ~.
\end{equation}

\begin{proof}[Proof of Claim~\ref{claim:invariant}]
Let 
\[ Q_i = S'^{i+1} \cup \left( C_i^\ast \cap \bigcup_{j=i+1}^\eta D_r^j\right).\]
By the definition of $C^*_{i+1}$, we have 
\[\cost(\calC + C^*_{i+1}) \leq \cost(\calC + Q_i),\] so it is sufficient to prove that 
\[\cost(\calC + Q_i) - \cost(\calC + C^*_i) \leq 4 \eta^{-2} |D(r)| \cdot |N(r)|.\]

We observe that 
\[ \cost(\calC + Q_i) - \cost(\calC + C^*_i) \leq  |Q_i \oplus C^*_i|^2 + \sum_{v \in Q_i \oplus C^*_i}\left(\cost(\calC + Q_i, v) - \cost(\calC + C^*_i, v)\right),\]
where $\oplus$ is the operation that computes the symmetric difference of two sets. 
Fix a vertex $v \in Q_i \oplus C^*_i$ and let $C \in \calC$ be the cluster containing $v$.
We have 
\[\cost(\calC + Q_i, v) - \cost(\calC + C^*_i, v) \leq |C| + |Q_i| + |C^*_i|.\]
According to Lemma~\ref{lem:bounded-minus-cost}, $|C| \leq 12\epsilon^{-4}d(v) \leq 24\epsilon^{-6}|N(r)|$. 
Since $Q_i, C^*_i$ are subsets of $N(r)$, $|Q_i| \leq |N(r)|$, $|C^*_i| \leq |N(r)|$, therefore 
\[\cost(\calC + Q_i, v) - \cost(\calC + C^*_i, v) \leq |C| + |Q_i| + |C^*_i| \leq 26\epsilon^{-6}|N(r)|.\]

We will be using chernoff bound for vertices
$v \in N(r)$. Note that if $v \in N(r)$, then by Claim~\ref{claim:degree},
\begin{equation}\label{eq:concentration-crap}
d^{\adm}(v) + |C(v)| + |K(r)| \leq 2d^{\adm}(v) + |N(r)| \leq 9\epsilon^{-5} |N(r)|.
\end{equation}

A vertex $v \in Q_i \oplus C^*_i$ can be one of the following three types. 
\begin{itemize}
    \item $v$ is a \emph{missing} node if $v \in Q_i$ and $v \notin C^*_i$. 
    \item $v$ is a \emph{core} node if $v \in C^*_i, v \notin Q_i$ and 
    \[ \rmCostMoves(C^*_i,v) +\eta^{-2} (9\epsilon^{-5}+1) |N(r)| < \rmCostStays(C^*_i,v). \]
    \item $v$ is a \emph{non-core} node if $v \in C^*_i, v \notin Q_i$ and \[ \rmCostMoves(C^*_i,v) +\eta^{-2} (9\epsilon^{-5}+1) |N(r)| \geq \rmCostStays(C^*_i,v). \]
\end{itemize}

In the following part, we will split the cost difference into vertices of the three types, and give a bound separately. 

\textbf{Missing nodes.} If $v \notin C^*_i$, by definition of $C^*_i$, $\rmCostMoves(C^*_i,v) \geq \rmCostStays(C^*_i,v)$. 
According to chernoff bound, with probability at most 
$2^{-\eta^2}$, we have
\[\rmEstCostMoves(C^*_i,v) + \eta^{-2} \cdot 9\epsilon^{-5} |N(r)| < \rmEstCostStays(C^*_i,v).\]
Therefore $v \in Q_i$ with probability at most $2^{-\eta^2}$,
so the expected size of $Q_i \setminus C^*_i$ is
bounded by $|D(r)| 2^{-\eta^2}$. 
Hence, there are more than $|D(r)| 2^{-\eta^2/2}$
missing nodes with probability at most $2^{-\eta^2/2}$. 
\mpcom{I have a problem here.
The conclustion $v \in Q_i$ does not match
the gap  $+\eta^{-3} s_i$ in the algorithm outline earlier.
I am not sure how to fix it. The same problem appears in the core node case below.}
\hwcom{I forget that. So we can use $\eta^{-1}s_i$ in the statement of the algorithm instead. Fixed. By the way, why do we use $\eta^{-2}(9\epsilon^{-5}+1)|N(r)|$ as the gap, I think $\eta^{-2}|N(r)|$ works well, and it's also easier to get a Chernoff bound. }
\mpcom{I am not sure $\eta^{-2}|N(r)|$ works. You need
to fit in somewhere the gap between $\rmEstCostMoves$
and $\rmCostMoves$, which can be as large as the expression
of~\eqref{eq:concentration-crap} times $\eta^{-2}$.}

\textbf{Core nodes.} If $v \in C^*_i$ is a core node,
according to chernoff bound %
we have
\[\rmEstCostMoves(C^*_i,v) + \eta^{-2}|N(r)| \geq \rmEstCostStays(C^*_i,v)\]
with probability at most $2^{-\eta^2}$.
Therefore $v \notin Q_i$ with probability at most $2^{-\eta^2}$. 
Similarly as before, 
there are at most $|D(r)| 2^{-\eta^2/2}$ core vertices with probability at least $1 - 2^{-\eta^2/2}$.

\textbf{Non-core nodes.} If $v \in C^*_i$ is a non-core node, 
then 
\begin{align*}
 &\cost(\calC + Q_i, v) - \cost(\calC + C^*_i, v) \\
 &\qquad \leq \rmCostStays(C^*_i, v) - \rmCostMoves(C^*_i, v) + |Q_i \oplus C^*_i| \\
 &\qquad \leq \eta^{-2}(9\epsilon^{-5} + 1)|N(r)| + \eta^{-1}|D(r)| \leq 2\eta^{-1} |N(r)|. 
\end{align*}
In the last inequality we used the fact that
$Q_i \oplus C_i^\ast \subseteq D_i^r$ and $|D_i^r| = \eta^{-1} |D(r)|$.

Summing up the total cost difference over all vertices of the three types, we have
\begin{align*}
    &\cost(\calC + Q_i) - \cost(\calC + C^*_i) \\
    &\qquad \leq |Q_i \oplus C_i^\ast|^2 + \sum_{v \in Q_i \oplus C^*_i}\left(\cost(\calC + Q_i, v) - \cost(\calC + C^*_i, v)\right) \\
    &\qquad \leq \eta^{-2} |D(r)|^2 + 2 \cdot |D(r)| 2^{-\eta^2/2} \cdot 26 \epsilon^{-6} |N(r)| 
    + \eta^{-1} |D(r)| \cdot 2\eta^{-1} |N(r)| \\
    &\qquad \leq 4\eta^{-2} |D(r)| \cdot |N(r)|.
\end{align*}
This finishes the proof of the claim.
\end{proof}
This finishes the proof of the lemma.
\end{proof}

\include{near-linear-tools}


